The First Data Release from SweetSpot: 74 Supernovae in 36 Nights on WIYN+WHIRC

SweetSpot is a three-year National Optical Astronomy Observatory (NOAO) Survey program to observe Type Ia supernovae (SNe Ia) in the smooth Hubble flow with the WIYN High-resolution Infrared Camera (WHIRC) on the WIYN 3.5-m telescope. We here present data from the first half of this survey, covering the 2011B-2013B NOAO semesters, and consisting of 493 calibrated images of 74 SNe Ia observed in the rest-frame near-infrared (NIR) from $0.02 < z < 0.09$. Because many observed supernovae require host galaxy subtraction from templates taken in later semesters, this release contains only the 186 NIR ($JHK_s$) data points for the 33 SNe Ia that do not require host-galaxy subtraction. The sample includes 4 objects with coverage beginning before the epoch of B-band maximum and 27 beginning within 20 days of B-band maximum. We also provide photometric calibration between the WIYN+WHIRC and Two-Micron All Sky Survey (2MASS) systems along with light curves for 786 2MASS stars observed alongside the SNe Ia. This work is the first in a planned series of three SweetSpot Data Releases. Future releases will include the full set of images from all 3 years of the survey, including host-galaxy reference images and updated data processing and host-galaxy reference subtraction. SweetSpot will provide a well-calibrated sample that will help improve our ability to standardize distance measurements to SNe Ia, examine the intrinsic optical-NIR colors of SNe Ia at different epochs, explore nature of dust in other galaxies, and act as a stepping stone for more distant, potentially space-based surveys.

==> SNIa_lightcurves.tex <==
\begin{deluxetable}{lrrlrrrr}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
\tablecaption{SweetSpot Lightcurves\label{table:lightcurves}}
\tablehead{\colhead{Name} & \colhead{mjd} & \colhead{approxPhase} & \colhead{filter\tablenotemark{a}} & \colhead{mag} & \colhead{magErr} & \colhead{flux\tablenotemark{b}} & \colhead{fluxErr}}  % \colhead{ } & \colhead{$\mathrm{d}$} & \colhead{$\mathrm{d}$} & \colhead{ } & \colhead{$\mathrm{mag}$} & \colhead{$\mathrm{mag}$} & \colhead{ } & \colhead{ }}
\startdata
CSS121009:011101-172841 & 56234.27359 & 14.27359 & WHIRCJ & 18.97756 & 0.05157 & 256.4340 & 12.1698 \\
CSS121009:011101-172841 & 56229.31361 & 9.31361 & WHIRCH & 18.64361 & 0.04781 & 348.7850 & 15.3479 \\
CSS121009:011101-172841 & 56229.28541 & 9.28541 & WHIRCJ & 19.27324 & 0.07101 & 195.3014 & 12.7551 \\
CSS121009:011101-172841 & 56234.22657 & 14.22657 & WHIRCH & 18.53778 & 0.04162 & 384.4939 & 14.7330 \\
CSS121114:090202+101800 & 56254.50847 & 2.50847 & WHIRCH & 18.08766 & 0.02963 & 582.0156 & 15.8819 \\
CSS121114:090202+101800 & 56257.45088 & 5.45088 & WHIRCH & 18.29991 & 0.02746 & 478.6713 & 12.1028 \\
CSS121114:090202+101800 & 56262.48385 & 10.48385 & WHIRCH & 18.39446 & 0.03869 & 438.7490 & 15.6268 \\
CSS121114:090202+101800 & 56254.52481 & 2.52481 & WHIRCJ & 18.39741 & 0.02063 & 437.5576 & 8.3115 \\
CSS121114:090202+101800 & 56257.46387 & 5.46387 & WHIRCJ & 18.84659 & 0.02922 & 289.3104 & 7.7855 \\
CSS121114:090202+101800 & 56262.49573 & 10.49573 & WHIRCJ & 19.18741 & 0.04400 & 211.3655 & 8.5610 \\
LSQ12fhs & 56229.18441 & 14.18441 & WHIRCH & 17.62670 & 0.04234 & 889.8578 & 34.6828 \\
LSQ12fhs & 56262.09874 & 47.09874 & WHIRCJ & 19.29963 & 0.05243 & 190.6111 & 9.1971 \\
LSQ12fhs & 56254.09366 & 39.09366 & WHIRCJ & 19.07615 & 0.05002 & 234.1756 & 10.7798 \\
LSQ12fhs & 56234.19517 & 19.19517 & WHIRCJ & 18.20453 & 0.02412 & 522.6215 & 11.6097 \\
LSQ12fhs & 56229.20190 & 14.20190 & WHIRCJ & 18.10289 & 0.04167 & 573.9127 & 22.0156 \\
LSQ12fhs & 56262.06478 & 47.06478 & WHIRCH & 18.74395 & 0.07230 & 317.9950 & 21.1452 \\
LSQ12fhs & 56254.11603 & 39.11603 & WHIRCH & 18.39693 & 0.04528 & 437.7520 & 18.2472 \\
LSQ12fhs & 56234.18017 & 19.18017 & WHIRCH & 17.71930 & 0.03340 & 817.1110 & 25.1270 \\
LSQ12fmx & 56229.35056 & 2.35056 & WHIRCH & 19.36719 & 0.04266 & 179.1119 & 7.0333 \\
LSQ12fmx & 56257.27331 & 30.27331 & WHIRCH & 19.59783 & 0.04753 & 144.8337 & 6.3364 \\
LSQ12fmx & 56262.34668 & 35.34668 & WHIRCH & 19.83690 & 0.11267 & 116.2093 & 12.0162 \\
LSQ12fmx & 56229.39756 & 2.39756 & WHIRCJ & 19.29668 & 0.03715 & 191.1294 & 6.5379 \\
LSQ12fmx & 56234.38407 & 7.38407 & WHIRCH & 19.96764 & 0.09762 & 103.0255 & 9.2385 \\
LSQ12fmx & 56234.43086 & 7.43086 & WHIRCJ & 19.95668 & 0.09658 & 104.0702 & 9.2334 \\
LSQ13cmt & 56584.31926 & 9.31926 & WHIRCH & 18.18813 & 0.04625 & 530.5772 & 22.5891 \\
LSQ13cmt & 56581.28436 & 6.28436 & WHIRCJ & 17.99420 & 0.02952 & 634.3391 & 17.2411 \\
LSQ13cmt & 56586.32803 & 11.32803 & WHIRCJ & 18.80891 & 0.06029 & 299.5273 & 16.6163 \\
LSQ13cmt & 56586.30561 & 11.30561 & WHIRCH & 18.35185 & 0.05018 & 456.3114 & 21.0734 \\
LSQ13cmt & 56581.26194 & 6.26194 & WHIRCH & 18.03593 & 0.03894 & 610.4191 & 21.8811 \\
LSQ13cwp & 56617.29790 & 11.29790 & WHIRCJ & 19.48204 & 0.08557 & 161.1329 & 12.6736 \\
LSQ13cwp & 56608.42282 & 2.42282 & WHIRCJ & 18.65466 & 0.04892 & 345.2521 & 15.5457 \\
LSQ13cwp & 56640.28729 & 34.28729 & WHIRCJ & 19.42432 & 0.07656 & 169.9309 & 11.9625 \\
LSQ13cwp & 56640.26270 & 34.26270 & WHIRCH & 19.05540 & 0.09231 & 238.6924 & 20.2450 \\
LSQ13cwp & 56617.21589 & 11.21589 & WHIRCH & 18.86661 & 0.09072 & 284.0236 & 23.6771 \\
LSQ13cwp & 56608.38579 & 2.38579 & WHIRCH & 18.72881 & 0.06739 & 322.4610 & 19.9895 \\
LSQ13cwp & 56636.36635 & 30.36635 & WHIRCJ & 20.30477 & 0.25482 & 75.5255 & 17.4069 \\
PS1-13dkh & 56584.43367 & 12.43367 & WHIRCH & 17.51395 & 0.01467 & 987.2354 & 13.3347 \\
PS1-13dkh & 56608.33839 & 36.33839 & WHIRCH & 17.63576 & 0.01837 & 882.4650 & 14.9275 \\
PS1-13dkh & 56584.44199 & 12.44199 & WHIRCJ & 18.34259 & 0.01582 & 460.2196 & 6.7042 \\
PS1-13dkh & 56608.35287 & 36.35287 & WHIRCJ & 18.19634 & 0.02087 & 526.5785 & 10.1212 \\
PS1-13dkh & 56636.19904 & 64.19904 & WHIRCJ & 19.59913 & 0.10234 & 144.6604 & 13.5949 \\
PS1-13dkh & 56636.18417 & 64.18417 & WHIRCH & 18.68953 & 0.16637 & 334.3385 & 50.8355 \\
PTF11moy & 55860.11461 & 36.11461 & WHIRCJ & 20.09368 & 0.14560 & 91.7337 & 12.2286 \\
PTF11moy & 55860.13251 & 36.13251 & WHIRCH & 19.70119 & 0.19383 & 131.6817 & 23.2622 \\
PTF11qmo & 55904.49490 & 10.49490 & WHIRCJ & 19.64726 & 0.06919 & 138.3871 & 8.8072 \\
PTF11qmo & 55935.37799 & 41.37799 & WHIRCH & 18.84237 & 0.08181 & 290.4358 & 21.8422 \\
PTF11qmo & 55904.47779 & 10.47779 & WHIRCH & 18.83034 & 0.04674 & 293.6733 & 12.6352 \\
PTF11qmo & 55935.40492 & 41.40492 & WHIRCJ & 19.68551 & 0.11437 & 133.5966 & 14.0211 \\
PTF13asv & 56435.39767 & 12.39767 & WHIRCH & 17.79877 & 0.02485 & 759.4365 & 17.3780 \\
PTF13asv & 56441.37773 & 18.37773 & WHIRCH & 18.10286 & 0.03891 & 573.9267 & 20.5603 \\
PTF13asv & 56461.36792 & 38.36792 & WHIRCH & 17.66586 & 0.01824 & 858.3299 & 14.4163 \\
PTF13asv & 56457.39626 & 34.39626 & WHIRCH & 17.73282 & 0.04213 & 806.9986 & 31.3011 \\
PTF13dad & 56586.45366 & 39.45366 & WHIRCJ & 27.31938 & 0.64982 & 0.1181 & 0.0633 \\
PTF13dad & 56581.40990 & 34.40990 & WHIRCJ & 27.07142 & 0.64941 & 0.1484 & 0.0795 \\
PTF13dad & 56586.40905 & 39.40905 & WHIRCH & 20.22360 & 0.04854 & 81.3877 & 3.6359 \\
PTF13dad & 56581.35978 & 34.35978 & WHIRCH & 19.80473 & 0.04236 & 119.7036 & 4.6675 \\
PTF13dad & 56561.31567 & 14.31567 & WHIRCH & 20.22134 & 0.05480 & 81.5578 & 4.1130 \\
PTF13ddg & 56585.38618 & 40.38618 & WHIRCH & 20.01846 & 0.08013 & 98.3138 & 7.2426 \\
PTF13ddg & 56581.18817 & 36.18817 & WHIRCH & 19.84544 & 0.05608 & 115.2985 & 5.9501 \\
PTF13ddg & 56561.17936 & 16.17936 & WHIRCH & 19.09255 & 0.09158 & 230.6639 & 19.4101 \\
SN2011fe & 55860.07135 & 46.07135 & WHIRCK & 12.37023 & 0.06591 & 112696.3170 & 6833.3573 \\
SN2011fe & 56020.49175 & 206.49175 & WHIRCJ & 17.96930 & 0.05134 & 649.0554 & 30.6680 \\
SN2011fe & 55860.07410 & 46.07410 & WHIRCJ & 13.08258 & 0.04065 & 58474.4566 & 2188.0533 \\
SN2011fe & 55860.06579 & 46.06579 & WHIRCH & 11.91697 & 0.03557 & 171084.6261 & 5603.5862 \\
SN2011fe & 56020.48346 & 206.48346 & WHIRCH & 17.89705 & 0.04836 & 693.7143 & 30.8798 \\
SN2011fs & 55860.30238 & 27.30238 & WHIRCJ & 17.13283 & 0.02471 & 1402.3927 & 31.9160 \\
SN2011fs & 55881.14001 & 48.14001 & WHIRCH & 16.97204 & 0.01474 & 1626.2418 & 22.0707 \\
SN2011fs & 55860.29276 & 27.29276 & WHIRCH & 16.14016 & 0.01675 & 3498.9376 & 53.9622 \\
SN2011fs & 55881.16411 & 48.16411 & WHIRCJ & 17.73779 & 0.01826 & 803.3107 & 13.5064 \\
SN2011fs & 55904.09285 & 71.09285 & WHIRCH & 17.77224 & 0.02872 & 778.2218 & 20.5774 \\
SN2011fs & 55904.11262 & 71.11262 & WHIRCJ & 19.21216 & 0.04188 & 206.6021 & 7.9659 \\
SN2011fs & 55860.31167 & 27.31167 & WHIRCK & 16.32620 & 0.06342 & 2947.9490 & 172.0056 \\
SN2011fs & 55935.09024 & 102.09024 & WHIRCJ & 20.41071 & 0.21649 & 68.5043 & 13.4813 \\
SN2011fs & 55935.06171 & 102.06171 & WHIRCH & 18.74504 & 0.07551 & 317.6762 & 22.0590 \\
SN2011gf & 55860.22490 & 33.22490 & WHIRCH & 17.32946 & 0.04498 & 1170.0812 & 48.4463 \\
SN2011gf & 55881.05948 & 54.05948 & WHIRCH & 17.96596 & 0.03303 & 651.0534 & 19.7979 \\
SN2011gf & 55904.05770 & 77.05770 & WHIRCH & 18.77189 & 0.16387 & 309.9150 & 46.4227 \\
SN2011gf & 55860.21079 & 33.21079 & WHIRCJ & 18.33066 & 0.04367 & 465.3028 & 18.7047 \\
SN2011gf & 55881.07449 & 54.07449 & WHIRCJ & 19.13042 & 0.04104 & 222.7566 & 8.4169 \\
SN2011io & 55904.15409 & 10.15409 & WHIRCJ & 19.14274 & 0.04703 & 220.2432 & 9.5348 \\
SN2011io & 55904.13970 & 10.13970 & WHIRCH & 18.73809 & 0.04444 & 319.7168 & 13.0789 \\
SN2011iy & 56020.36359 & 124.36359 & WHIRCH & 17.24135 & 0.05255 & 1269.0003 & 61.3719 \\
SN2011iy & 56020.38029 & 124.38029 & WHIRCJ & 18.24914 & 0.09101 & 501.5825 & 41.9459 \\
SN2011jh & 56020.33161 & 91.33161 & WHIRCH & 18.67751 & 0.17576 & 338.0610 & 54.2536 \\
SN2011jh & 56020.34863 & 91.34863 & WHIRCJ & 20.43959 & 0.56186 & 66.7057 & 31.7362 \\
SN2012bh & 56020.27066 & 4.27066 & WHIRCH & 17.27685 & 0.01679 & 1228.1745 & 18.9957 \\
SN2012bh & 56020.27890 & 4.27890 & WHIRCJ & 17.22727 & 0.01548 & 1285.5605 & 18.3324 \\
SN2012bo & 56020.40244 & -0.59756 & WHIRCH & 16.37131 & 0.04600 & 2827.9797 & 119.7405 \\
SN2012bo & 56020.40716 & -0.59284 & WHIRCJ & 16.43152 & 0.03139 & 2675.4170 & 77.3249 \\
SN2012bp & 56020.51105 & 7.51105 & WHIRCJ & 17.73159 & 0.02630 & 807.9143 & 19.5665 \\
SN2012bp & 56020.50536 & 7.50536 & WHIRCH & 17.51160 & 0.02206 & 989.3704 & 20.0956 \\
SN2012em & 56196.21274 & 15.21274 & WHIRCJ & 18.97292 & 0.03439 & 257.5320 & 8.1553 \\
SN2012em & 56196.18464 & 15.18464 & WHIRCH & 18.58777 & 0.04301 & 367.1903 & 14.5369 \\
SN2012fk & 56234.32294 & 11.32294 & WHIRCH & 17.83844 & 0.01879 & 732.1888 & 12.6733 \\
SN2012fk & 56257.22896 & 34.22896 & WHIRCH & 18.70868 & 0.03667 & 328.4954 & 11.0898 \\
SN2012fk & 56262.29933 & 39.29933 & WHIRCH & 19.09234 & 0.03433 & 230.7093 & 7.2915 \\
SN2012fk & 56234.33988 & 11.33988 & WHIRCJ & 18.67895 & 0.02360 & 337.6132 & 7.3387 \\
SN2012fk & 56257.24358 & 34.24358 & WHIRCJ & 19.40700 & 0.05636 & 172.6626 & 8.9547 \\
SN2012fr & 56234.30669 & -5.69331 & WHIRCH & 13.30711 & 0.03665 & 47550.7993 & 1604.6337 \\
SN2012fr & 56234.31523 & -5.68477 & WHIRCJ & 13.02204 & 0.03573 & 61827.9113 & 2033.7157 \\
SN2013ar & 56378.18000 & 4.18000 & WHIRCJ & 21.61015 & 0.32937 & 22.6955 & 6.6812 \\
SN2013ar & 56378.14022 & 4.14022 & WHIRCH & 21.41520 & 0.37869 & 27.1595 & 9.1066 \\
SN2013ar & 56403.13002 & 29.13002 & WHIRCH & 21.56730 & 0.55557 & 23.6092 & 11.1263 \\
SN2013ar & 56412.18302 & 38.18302 & WHIRCJ & 22.13422 & 0.46178 & 14.0059 & 5.6220 \\
SN2013ar & 56412.14117 & 38.14117 & WHIRCH & 21.29545 & 0.49868 & 30.3263 & 13.0255 \\
SN2013bs & 56435.47398 & 32.47398 & WHIRCJ & 18.45282 & 0.05032 & 415.7894 & 19.2559 \\
SN2013bs & 56457.46418 & 54.46418 & WHIRCJ & 20.31953 & 0.27680 & 74.5051 & 18.5933 \\
SN2013bs & 56441.44940 & 38.44940 & WHIRCJ & 18.96375 & 0.05364 & 259.7171 & 12.8201 \\
SN2013bs & 56408.49228 & 5.49228 & WHIRCJ & 16.74712 & 0.01200 & 2000.5699 & 22.1052 \\
SN2013bs & 56403.46082 & 0.46082 & WHIRCJ & 16.76254 & 0.01286 & 1972.3511 & 23.3677 \\
SN2013bs & 56461.41814 & 58.41814 & WHIRCH & 18.89789 & 0.06191 & 275.9585 & 15.7185 \\
SN2013bs & 56457.44571 & 54.44571 & WHIRCH & 19.08329 & 0.12021 & 232.6396 & 25.6530 \\
SN2013bs & 56441.43318 & 38.43318 & WHIRCH & 18.51243 & 0.05293 & 393.5743 & 19.1729 \\
SN2013bs & 56435.46406 & 32.46406 & WHIRCH & 18.02158 & 0.04304 & 618.5421 & 24.5078 \\
SN2013bs & 56412.47950 & 9.47950 & WHIRCH & 17.69737 & 0.02885 & 833.7791 & 22.1528 \\
SN2013bs & 56408.48689 & 5.48689 & WHIRCH & 16.62438 & 0.01463 & 2239.9937 & 30.1722 \\
SN2013bs & 56403.44112 & 0.44112 & WHIRCH & 16.86693 & 0.01446 & 1791.5430 & 23.8549 \\
SN2013bs & 56461.44315 & 58.44315 & WHIRCJ & 21.01270 & 0.27460 & 39.3479 & 9.7447 \\
SN2013bt & 56412.42546 & 4.42546 & WHIRCJ & 17.55214 & 0.02276 & 953.1097 & 19.9802 \\
SN2013bt & 56436.38252 & 28.38252 & WHIRCJ & 18.73328 & 0.05757 & 321.1367 & 17.0117 \\
SN2013bt & 56403.40590 & -4.59410 & WHIRCH & 17.75819 & 0.02989 & 788.3565 & 21.7001 \\
SN2013bt & 56408.45670 & 0.45670 & WHIRCH & 17.49899 & 0.02014 & 1000.9329 & 18.5615 \\
SN2013bt & 56412.40951 & 4.40951 & WHIRCH & 17.76281 & 0.02788 & 785.0121 & 20.1564 \\
SN2013bt & 56432.30787 & 24.30787 & WHIRCH & 17.59589 & 0.02087 & 915.4710 & 17.5974 \\
SN2013bt & 56436.35763 & 28.35763 & WHIRCH & 18.00003 & 0.03991 & 630.9377 & 23.1831 \\
SN2013bt & 56408.44833 & 0.44833 & WHIRCJ & 17.27991 & 0.01656 & 1224.7126 & 18.6828 \\
SN2013bt & 56432.33212 & 24.33212 & WHIRCJ & 18.19832 & 0.02412 & 525.6201 & 11.6748 \\
SN2013bt & 56403.42458 & -4.57542 & WHIRCJ & 17.58586 & 0.02237 & 923.9693 & 19.0378 \\
SN2013cs & 56441.15469 & 5.15469 & WHIRCH & 14.71889 & 0.01570 & 12955.2055 & 187.2833 \\
SN2013cs & 56457.15867 & 21.15867 & WHIRCH & 14.57409 & 0.01564 & 14803.4860 & 213.2374 \\
SN2013cs & 56461.15182 & 25.15182 & WHIRCH & 14.50506 & 0.01564 & 15775.2935 & 227.2892 \\
SN2013cs & 56436.15128 & 0.15128 & WHIRCJ & 14.28690 & 0.01597 & 19285.8728 & 283.7246 \\
SN2013cs & 56441.16450 & 5.16450 & WHIRCJ & 14.62909 & 0.01612 & 14072.2078 & 208.9566 \\
SN2013cs & 56457.16921 & 21.16921 & WHIRCJ & 15.83277 & 0.01666 & 4644.0032 & 71.2681 \\
SN2013cs & 56461.16252 & 25.16252 & WHIRCJ & 15.62282 & 0.01664 & 5634.6998 & 86.3731 \\
SN2013cs & 56436.16145 & 0.16145 & WHIRCH & 14.56148 & 0.01562 & 14976.3730 & 215.4565 \\
SN2013fn & 56581.10267 & 9.10267 & WHIRCH & 17.52947 & 0.02097 & 973.2240 & 18.7976 \\
SN2013fn & 56586.05958 & 14.05958 & WHIRCH & 17.47423 & 0.02401 & 1024.0205 & 22.6391 \\
SN2013fn & 56608.05876 & 36.05876 & WHIRCH & 17.51843 & 0.02718 & 983.1658 & 24.6066 \\
SN2013fn & 56581.11308 & 9.11308 & WHIRCJ & 17.98581 & 0.02212 & 639.2556 & 13.0228 \\
SN2013fn & 56586.06894 & 14.06894 & WHIRCJ & 18.46028 & 0.03267 & 412.9421 & 12.4225 \\
SN2013fn & 56608.07328 & 36.07328 & WHIRCJ & 17.99965 & 0.03069 & 631.1582 & 17.8366 \\
SN2013fn & 56581.12161 & 9.12161 & WHIRCK & 17.11799 & 0.03851 & 1421.6874 & 50.4095 \\
SN2013fn & 56586.07718 & 14.07718 & WHIRCK & 17.18156 & 0.03487 & 1340.8373 & 43.0513 \\
iPTF13dge & 56591.50141 & 36.50141 & WHIRCH & 16.52956 & 0.01312 & 2444.4147 & 29.5352 \\
iPTF13dge & 56586.50377 & 31.50377 & WHIRCH & 16.00029 & 0.01186 & 3979.9989 & 43.4850 \\
iPTF13dge & 56584.40566 & 29.40566 & WHIRCH & 15.87628 & 0.01146 & 4461.5861 & 47.0733 \\
iPTF13dge & 56608.46109 & 53.46109 & WHIRCH & 17.66258 & 0.01806 & 860.9338 & 14.3213 \\
iPTF13dge & 56563.49315 & 8.49315 & WHIRCH & 16.56236 & 0.01296 & 2371.6740 & 28.3000 \\
iPTF13dge & 56636.40312 & 81.40312 & WHIRCH & 18.34840 & 0.05755 & 457.7643 & 24.2431 \\
iPTF13dge & 56581.47155 & 26.47155 & WHIRCH & 16.03264 & 0.01190 & 3863.1807 & 42.3400 \\
iPTF13dge & 56640.33546 & 85.33546 & WHIRCH & 18.93797 & 0.06199 & 265.9562 & 15.1686 \\
iPTF13dge & 56581.47993 & 26.47993 & WHIRCJ & 17.24511 & 0.01383 & 1264.6121 & 16.1025 \\
iPTF13dge & 56640.37611 & 85.37611 & WHIRCK & 18.61907 & 0.10671 & 356.7577 & 34.9522 \\
iPTF13dge & 56636.43949 & 81.43949 & WHIRCK & 18.94088 & 0.56826 & 265.2452 & 127.4000 \\
iPTF13dge & 56563.50245 & 8.50245 & WHIRCJ & 16.83884 & 0.01332 & 1838.4976 & 22.5552 \\
iPTF13dge & 56586.52030 & 31.52030 & WHIRCK & 16.12456 & 0.01883 & 3549.5575 & 61.5663 \\
iPTF13dge & 56584.41948 & 29.41948 & WHIRCK & 15.77992 & 0.01623 & 4875.6274 & 72.8552 \\
iPTF13dge & 56581.48814 & 26.48814 & WHIRCK & 16.00012 & 0.01717 & 3980.6335 & 62.9567 \\
iPTF13dge & 56591.50969 & 36.50969 & WHIRCK & 16.54262 & 0.02088 & 2415.2024 & 46.4452 \\
iPTF13dge & 56636.41890 & 81.41890 & WHIRCJ & 20.38050 & 0.17157 & 70.4370 & 11.0389 \\
iPTF13dge & 56608.48582 & 53.48582 & WHIRCJ & 19.27159 & 0.04326 & 195.5981 & 7.7894 \\
iPTF13dge & 56591.52441 & 36.52441 & WHIRCJ & 17.42516 & 0.01332 & 1071.3620 & 13.1428 \\
iPTF13dge & 56586.51208 & 31.51208 & WHIRCJ & 16.95876 & 0.01263 & 1646.2577 & 19.1422 \\
iPTF13dge & 56640.35126 & 85.35126 & WHIRCJ & 20.65380 & 0.19175 & 54.7623 & 9.5724 \\
iPTF13dge & 56584.41120 & 29.41120 & WHIRCJ & 16.84558 & 0.01234 & 1827.1158 & 20.7615 \\
iPTF13dkl & 56563.36130 & 7.36130 & WHIRCH & 18.56847 & 0.05115 & 373.7778 & 17.5948 \\
iPTF13dkl & 56584.34696 & 28.34696 & WHIRCH & 18.70421 & 0.04635 & 329.8484 & 14.0719 \\
iPTF13dkl & 56563.36951 & 7.36951 & WHIRCJ & 18.03202 & 0.02954 & 612.6198 & 16.6651 \\
iPTF13dkl & 56584.36493 & 28.36493 & WHIRCJ & 19.32750 & 0.07278 & 185.7799 & 12.4340 \\
iPTF13dkx & 56581.24375 & 20.24375 & WHIRCJ & 18.64006 & 0.02005 & 349.9251 & 6.4609 \\
iPTF13dkx & 56585.34448 & 24.34448 & WHIRCH & 17.54054 & 0.01941 & 963.3520 & 17.2241 \\
iPTF13dkx & 56581.23899 & 20.23899 & WHIRCH & 17.44612 & 0.01859 & 1050.8792 & 17.9887 \\
iPTF13dkx & 56563.42330 & 2.42330 & WHIRCJ & 17.16061 & 0.01971 & 1366.9592 & 24.8068 \\
iPTF13dkx & 56608.16421 & 47.16421 & WHIRCJ & 18.72205 & 0.02621 & 324.4736 & 7.8307 \\
iPTF13dkx & 56563.41323 & 2.41323 & WHIRCH & 17.38961 & 0.02056 & 1107.0185 & 20.9614 \\
iPTF13dkx & 56608.15223 & 47.15223 & WHIRCH & 17.97829 & 0.02146 & 643.7012 & 12.7196 \\
iPTF13ebh & 56636.14241 & 17.14241 & WHIRCH & 15.36282 & 0.03184 & 7159.3150 & 209.8877 \\
iPTF13ebh & 56640.14095 & 21.14095 & WHIRCH & 15.47487 & 0.01139 & 6457.3185 & 67.7338 \\
iPTF13ebh & 56617.14329 & -1.85671 & WHIRCJ & 15.40729 & 0.01294 & 6871.9917 & 81.8816 \\
iPTF13ebh & 56636.15130 & 17.15130 & WHIRCJ & 16.41932 & 0.04776 & 2705.6447 & 118.9459 \\
iPTF13ebh & 56640.15049 & 21.15049 & WHIRCJ & 16.22341 & 0.01276 & 3240.6910 & 38.0783 \\
iPTF13ebh & 56617.15312 & -1.84688 & WHIRCK & 15.39068 & 0.01739 & 6977.9267 & 111.7250 \\
iPTF13ebh & 56636.16017 & 17.16017 & WHIRCK & 15.48230 & 0.07114 & 6413.2790 & 419.6413 \\
iPTF13ebh & 56640.15936 & 21.15936 & WHIRCK & 15.45387 & 0.01509 & 6583.4459 & 91.4833 \\
iPTF13ebh & 56617.13733 & -1.86267 & WHIRCH & 15.47307 & 0.01356 & 6468.0416 & 80.7895 \\
\enddata

\tablenotetext{a}{
The WIYN+WHIRC $K_s$ filter is called ``WHIRCK'' in \code{SNooPy}'s system transmission database.
We adopt the SNooPy filter names here for future convenience.
}
\tablenotemark{b}{
Fluxes are given with respect to a zeropoint of 25: ${\rm mag}=-2.5\log_{10}({\rm flux}) + 25$.
}

\end{deluxetable}


==> SNIa_observations.tex <==
\begin{deluxetable}{llllrrl}
\tablecaption{Image Information\label{table:imageinfo}}
\tablehead{\colhead{Name} & \colhead{Set} & \colhead{Filter} & \colhead{Date\tablenotemark{a}} & \colhead{approxMjd} & \colhead{approxPhase} & \colhead{imageName}}  % \colhead{ } & \colhead{ } & \colhead{ } & \colhead{ } & \colhead{ } & \colhead{$\mathrm{d}$} & \colhead{ }}
\startdata
CSS121006:232854+085452 & A & H & 2012-10-28 & 56228 & 21 & CSS121006:232854+085452\_A\_H\_20121028.fits \\
CSS121006:232854+085452 & A & H & 2012-11-02 & 56233 & 26 & CSS121006:232854+085452\_A\_H\_20121102.fits \\
CSS121009:011101-172841 & A & H & 2012-10-28 & 56228 & 8 & CSS121009:011101-172841\_A\_H\_20121028.fits \\
CSS121009:011101-172841 & A & H & 2012-11-02 & 56233 & 13 & CSS121009:011101-172841\_A\_H\_20121102.fits \\
CSS121009:011101-172841 & A & J & 2012-10-28 & 56228 & 8 & CSS121009:011101-172841\_A\_J\_20121028.fits \\
CSS121009:011101-172841 & A & J & 2012-11-02 & 56233 & 13 & CSS121009:011101-172841\_A\_J\_20121102.fits \\
CSS121114:090202+101800 & A & H & 2012-11-22 & 56253 & 1 & CSS121114:090202+101800\_A\_H\_20121122.fits \\
CSS121114:090202+101800 & A & H & 2012-11-25 & 56256 & 4 & CSS121114:090202+101800\_A\_H\_20121125.fits \\
CSS121114:090202+101800 & A & H & 2012-11-30 & 56261 & 9 & CSS121114:090202+101800\_A\_H\_20121130.fits \\
CSS121114:090202+101800 & A & J & 2012-11-22 & 56253 & 1 & CSS121114:090202+101800\_A\_J\_20121122.fits \\
CSS121114:090202+101800 & A & J & 2012-11-25 & 56256 & 4 & CSS121114:090202+101800\_A\_J\_20121125.fits \\
CSS121114:090202+101800 & A & J & 2012-11-30 & 56261 & 9 & CSS121114:090202+101800\_A\_J\_20121130.fits \\
CSS130218:092354+385837 & A & H & 2013-03-26 & 56377 & 16 & CSS130218:092354+385837\_A\_H\_20130326.fits \\
CSS130218:092354+385837 & A & H & 2013-04-20 & 56402 & 41 & CSS130218:092354+385837\_A\_H\_20130420.fits \\
CSS130218:092354+385837 & A & H & 2013-04-25 & 56407 & 46 & CSS130218:092354+385837\_A\_H\_20130425.fits \\
CSS130317:082848+293031 & A & H & 2013-03-26 & 56377 & 7 & CSS130317:082848+293031\_A\_H\_20130326.fits \\
CSS130317:082848+293031 & A & H & 2013-04-20 & 56402 & 32 & CSS130317:082848+293031\_A\_H\_20130420.fits \\
CSS130317:082848+293031 & A & H & 2013-04-25 & 56407 & 37 & CSS130317:082848+293031\_A\_H\_20130425.fits \\
CSS130317:082848+293031 & A & J & 2013-03-26 & 56377 & 7 & CSS130317:082848+293031\_A\_J\_20130326.fits \\
CSS130317:082848+293031 & A & J & 2013-04-20 & 56402 & 32 & CSS130317:082848+293031\_A\_J\_20130420.fits \\
CSS130317:082848+293031 & A & J & 2013-04-25 & 56407 & 37 & CSS130317:082848+293031\_A\_J\_20130425.fits \\
LSQ12fhs & A & H & 2012-10-28 & 56228 & 13 & LSQ12fhs\_A\_H\_20121028.fits \\
LSQ12fhs & A & H & 2012-11-02 & 56233 & 18 & LSQ12fhs\_A\_H\_20121102.fits \\
LSQ12fhs & A & H & 2012-11-22 & 56253 & 38 & LSQ12fhs\_A\_H\_20121122.fits \\
LSQ12fhs & A & H & 2012-11-30 & 56261 & 46 & LSQ12fhs\_A\_H\_20121130.fits \\
LSQ12fhs & A & J & 2012-10-28 & 56228 & 13 & LSQ12fhs\_A\_J\_20121028.fits \\
LSQ12fhs & A & J & 2012-11-02 & 56233 & 18 & LSQ12fhs\_A\_J\_20121102.fits \\
LSQ12fhs & A & J & 2012-11-22 & 56253 & 38 & LSQ12fhs\_A\_J\_20121122.fits \\
LSQ12fhs & A & J & 2012-11-30 & 56261 & 46 & LSQ12fhs\_A\_J\_20121130.fits \\
LSQ12fmx & A & H & 2012-10-28 & 56228 & 1 & LSQ12fmx\_A\_H\_20121028.fits \\
LSQ12fmx & A & H & 2012-11-02 & 56233 & 6 & LSQ12fmx\_A\_H\_20121102.fits \\
LSQ12fmx & A & H & 2012-11-25 & 56256 & 29 & LSQ12fmx\_A\_H\_20121125.fits \\
LSQ12fmx & A & H & 2012-11-30 & 56261 & 34 & LSQ12fmx\_A\_H\_20121130.fits \\
LSQ12fmx & A & J & 2012-10-28 & 56228 & 1 & LSQ12fmx\_A\_J\_20121028.fits \\
LSQ12fmx & A & J & 2012-11-02 & 56233 & 6 & LSQ12fmx\_A\_J\_20121102.fits \\
LSQ12fmx & A & J & 2012-11-22 & 56253 & 26 & LSQ12fmx\_A\_J\_20121122.fits \\
LSQ12fuk & A & H & 2012-11-02 & 56233 & 1 & LSQ12fuk\_A\_H\_20121102.fits \\
LSQ12fuk & A & H & 2012-11-22 & 56253 & 21 & LSQ12fuk\_A\_H\_20121122.fits \\
LSQ12fuk & A & H & 2012-11-25 & 56256 & 24 & LSQ12fuk\_A\_H\_20121125.fits \\
LSQ12fuk & A & H & 2012-11-30 & 56261 & 29 & LSQ12fuk\_A\_H\_20121130.fits \\
LSQ12fuk & A & H & 2013-10-19 & 56584 & 352 & LSQ12fuk\_A\_H\_20131019.fits \\
LSQ12fuk & A & J & 2012-11-02 & 56233 & 1 & LSQ12fuk\_A\_J\_20121102.fits \\
LSQ12fuk & A & J & 2012-11-22 & 56253 & 21 & LSQ12fuk\_A\_J\_20121122.fits \\
LSQ12fuk & A & J & 2012-11-25 & 56256 & 24 & LSQ12fuk\_A\_J\_20121125.fits \\
LSQ12fuk & A & J & 2012-11-30 & 56261 & 29 & LSQ12fuk\_A\_J\_20121130.fits \\
LSQ12fuk & A & J & 2013-10-19 & 56584 & 352 & LSQ12fuk\_A\_J\_20131019.fits \\
LSQ12gef & A & H & 2012-11-22 & 56253 & 6 & LSQ12gef\_A\_H\_20121122.fits \\
LSQ12gef & A & H & 2012-11-25 & 56256 & 9 & LSQ12gef\_A\_H\_20121125.fits \\
LSQ12gef & A & H & 2012-11-30 & 56261 & 14 & LSQ12gef\_A\_H\_20121130.fits \\
LSQ12gef & A & J & 2012-11-22 & 56253 & 6 & LSQ12gef\_A\_J\_20121122.fits \\
LSQ12gef & A & J & 2012-11-25 & 56256 & 9 & LSQ12gef\_A\_J\_20121125.fits \\
LSQ13cmt & A & H & 2013-10-15 & 56580 & 5 & LSQ13cmt\_A\_H\_20131015.fits \\
LSQ13cmt & A & H & 2013-10-18 & 56583 & 8 & LSQ13cmt\_A\_H\_20131018.fits \\
LSQ13cmt & A & H & 2013-10-20 & 56585 & 10 & LSQ13cmt\_A\_H\_20131020.fits \\
LSQ13cmt & A & J & 2013-10-15 & 56580 & 5 & LSQ13cmt\_A\_J\_20131015.fits \\
LSQ13cmt & A & J & 2013-10-20 & 56585 & 10 & LSQ13cmt\_A\_J\_20131020.fits \\
LSQ13crf & A & H & 2013-11-11 & 56607 & 11 & LSQ13crf\_A\_H\_20131111.fits \\
LSQ13crf & A & H & 2013-12-09 & 56635 & 39 & LSQ13crf\_A\_H\_20131209.fits \\
LSQ13crf & A & H & 2013-12-13 & 56639 & 43 & LSQ13crf\_A\_H\_20131213.fits \\
LSQ13crf & A & J & 2013-11-11 & 56607 & 11 & LSQ13crf\_A\_J\_20131111.fits \\
LSQ13crf & A & J & 2013-12-09 & 56635 & 39 & LSQ13crf\_A\_J\_20131209.fits \\
LSQ13cwp & A & H & 2013-11-11 & 56607 & 1 & LSQ13cwp\_A\_H\_20131111.fits \\
LSQ13cwp & A & H & 2013-11-20 & 56616 & 10 & LSQ13cwp\_A\_H\_20131120.fits \\
LSQ13cwp & A & H & 2013-12-09 & 56635 & 29 & LSQ13cwp\_A\_H\_20131209.fits \\
LSQ13cwp & A & H & 2013-12-13 & 56639 & 33 & LSQ13cwp\_A\_H\_20131213.fits \\
LSQ13cwp & A & J & 2013-11-11 & 56607 & 1 & LSQ13cwp\_A\_J\_20131111.fits \\
LSQ13cwp & A & J & 2013-11-20 & 56616 & 10 & LSQ13cwp\_A\_J\_20131120.fits \\
LSQ13cwp & A & J & 2013-12-09 & 56635 & 29 & LSQ13cwp\_A\_J\_20131209.fits \\
LSQ13cwp & A & J & 2013-12-13 & 56639 & 33 & LSQ13cwp\_A\_J\_20131213.fits \\
P161-D & A & H & 2012-11-02 & 56233 & -- & P161-D\_A\_H\_20121102.fits \\
P161-D & A & H & 2012-11-22 & 56253 & -- & P161-D\_A\_H\_20121122.fits \\
P161-D & A & H & 2012-11-25 & 56256 & -- & P161-D\_A\_H\_20121125.fits \\
P161-D & A & H & 2012-11-30 & 56261 & -- & P161-D\_A\_H\_20121130.fits \\
P161-D & A & H & 2013-09-25 & 56560 & -- & P161-D\_A\_H\_20130925.fits \\
P161-D & A & H & 2013-09-27 & 56562 & -- & P161-D\_A\_H\_20130927.fits \\
P161-D & A & H & 2013-10-15 & 56580 & -- & P161-D\_A\_H\_20131015.fits \\
P161-D & A & H & 2013-10-18 & 56583 & -- & P161-D\_A\_H\_20131018.fits \\
P161-D & A & H & 2013-10-20 & 56585 & -- & P161-D\_A\_H\_20131020.fits \\
P161-D & A & H & 2013-11-11 & 56607 & -- & P161-D\_A\_H\_20131111.fits \\
P161-D & A & H & 2013-12-09 & 56635 & -- & P161-D\_A\_H\_20131209.fits \\
P161-D & A & H & 2013-12-13 & 56639 & -- & P161-D\_A\_H\_20131213.fits \\
P161-D & A & J & 2012-11-02 & 56233 & -- & P161-D\_A\_J\_20121102.fits \\
P161-D & A & J & 2012-11-22 & 56253 & -- & P161-D\_A\_J\_20121122.fits \\
P161-D & A & J & 2012-11-25 & 56256 & -- & P161-D\_A\_J\_20121125.fits \\
P161-D & A & J & 2012-11-30 & 56261 & -- & P161-D\_A\_J\_20121130.fits \\
P161-D & A & J & 2013-09-25 & 56560 & -- & P161-D\_A\_J\_20130925.fits \\
P161-D & A & J & 2013-09-27 & 56562 & -- & P161-D\_A\_J\_20130927.fits \\
P161-D & A & J & 2013-10-15 & 56580 & -- & P161-D\_A\_J\_20131015.fits \\
P161-D & A & J & 2013-10-18 & 56583 & -- & P161-D\_A\_J\_20131018.fits \\
P161-D & A & J & 2013-10-20 & 56585 & -- & P161-D\_A\_J\_20131020.fits \\
P161-D & A & J & 2013-11-11 & 56607 & -- & P161-D\_A\_J\_20131111.fits \\
P161-D & A & J & 2013-12-09 & 56635 & -- & P161-D\_A\_J\_20131209.fits \\
P161-D & A & J & 2013-12-13 & 56639 & -- & P161-D\_A\_J\_20131213.fits \\
P161-D & A & KS & 2012-11-22 & 56253 & -- & P161-D\_A\_KS\_20121122.fits \\
P161-D & A & KS & 2012-11-25 & 56256 & -- & P161-D\_A\_KS\_20121125.fits \\
P161-D & A & KS & 2012-11-30 & 56261 & -- & P161-D\_A\_KS\_20121130.fits \\
P161-D & A & KS & 2013-09-25 & 56560 & -- & P161-D\_A\_KS\_20130925.fits \\
P161-D & A & KS & 2013-09-27 & 56562 & -- & P161-D\_A\_KS\_20130927.fits \\
P161-D & A & KS & 2013-10-15 & 56580 & -- & P161-D\_A\_KS\_20131015.fits \\
P161-D & A & KS & 2013-10-18 & 56583 & -- & P161-D\_A\_KS\_20131018.fits \\
P161-D & A & KS & 2013-10-20 & 56585 & -- & P161-D\_A\_KS\_20131020.fits \\
P161-D & A & KS & 2013-11-11 & 56607 & -- & P161-D\_A\_KS\_20131111.fits \\
P161-D & A & KS & 2013-12-09 & 56635 & -- & P161-D\_A\_KS\_20131209.fits \\
P161-D & A & KS & 2013-12-13 & 56639 & -- & P161-D\_A\_KS\_20131213.fits \\
P161-D & B & H & 2012-11-25 & 56256 & -- & P161-D\_B\_H\_20121125.fits \\
P161-D & B & H & 2013-09-25 & 56560 & -- & P161-D\_B\_H\_20130925.fits \\
P161-D & B & H & 2013-09-27 & 56562 & -- & P161-D\_B\_H\_20130927.fits \\
P161-D & B & H & 2013-10-15 & 56580 & -- & P161-D\_B\_H\_20131015.fits \\
P161-D & B & H & 2013-10-18 & 56583 & -- & P161-D\_B\_H\_20131018.fits \\
P161-D & B & H & 2013-10-20 & 56585 & -- & P161-D\_B\_H\_20131020.fits \\
P161-D & B & H & 2013-11-11 & 56607 & -- & P161-D\_B\_H\_20131111.fits \\
P161-D & B & H & 2013-12-09 & 56635 & -- & P161-D\_B\_H\_20131209.fits \\
P161-D & B & H & 2013-12-13 & 56639 & -- & P161-D\_B\_H\_20131213.fits \\
P161-D & B & J & 2012-11-25 & 56256 & -- & P161-D\_B\_J\_20121125.fits \\
P161-D & B & J & 2013-09-25 & 56560 & -- & P161-D\_B\_J\_20130925.fits \\
P161-D & B & J & 2013-09-27 & 56562 & -- & P161-D\_B\_J\_20130927.fits \\
P161-D & B & J & 2013-10-15 & 56580 & -- & P161-D\_B\_J\_20131015.fits \\
P161-D & B & J & 2013-10-18 & 56583 & -- & P161-D\_B\_J\_20131018.fits \\
P161-D & B & J & 2013-10-20 & 56585 & -- & P161-D\_B\_J\_20131020.fits \\
P161-D & B & J & 2013-11-11 & 56607 & -- & P161-D\_B\_J\_20131111.fits \\
P161-D & B & J & 2013-12-09 & 56635 & -- & P161-D\_B\_J\_20131209.fits \\
P161-D & B & J & 2013-12-13 & 56639 & -- & P161-D\_B\_J\_20131213.fits \\
P161-D & B & KS & 2012-11-25 & 56256 & -- & P161-D\_B\_KS\_20121125.fits \\
P161-D & B & KS & 2013-09-25 & 56560 & -- & P161-D\_B\_KS\_20130925.fits \\
P161-D & B & KS & 2013-09-27 & 56562 & -- & P161-D\_B\_KS\_20130927.fits \\
P161-D & B & KS & 2013-10-15 & 56580 & -- & P161-D\_B\_KS\_20131015.fits \\
P161-D & B & KS & 2013-10-18 & 56583 & -- & P161-D\_B\_KS\_20131018.fits \\
P161-D & B & KS & 2013-10-20 & 56585 & -- & P161-D\_B\_KS\_20131020.fits \\
P161-D & B & KS & 2013-11-11 & 56607 & -- & P161-D\_B\_KS\_20131111.fits \\
P161-D & B & KS & 2013-12-09 & 56635 & -- & P161-D\_B\_KS\_20131209.fits \\
P161-D & B & KS & 2013-12-13 & 56639 & -- & P161-D\_B\_KS\_20131213.fits \\
P161-D & C & H & 2012-11-25 & 56256 & -- & P161-D\_C\_H\_20121125.fits \\
P161-D & C & H & 2013-09-25 & 56560 & -- & P161-D\_C\_H\_20130925.fits \\
P161-D & C & H & 2013-09-27 & 56562 & -- & P161-D\_C\_H\_20130927.fits \\
P161-D & C & H & 2013-10-15 & 56580 & -- & P161-D\_C\_H\_20131015.fits \\
P161-D & C & H & 2013-10-20 & 56585 & -- & P161-D\_C\_H\_20131020.fits \\
P161-D & C & J & 2012-11-25 & 56256 & -- & P161-D\_C\_J\_20121125.fits \\
P161-D & C & J & 2013-09-25 & 56560 & -- & P161-D\_C\_J\_20130925.fits \\
P161-D & C & J & 2013-09-27 & 56562 & -- & P161-D\_C\_J\_20130927.fits \\
P161-D & C & J & 2013-10-15 & 56580 & -- & P161-D\_C\_J\_20131015.fits \\
P161-D & C & J & 2013-10-20 & 56585 & -- & P161-D\_C\_J\_20131020.fits \\
P161-D & C & KS & 2013-09-25 & 56560 & -- & P161-D\_C\_KS\_20130925.fits \\
P161-D & C & KS & 2013-09-27 & 56562 & -- & P161-D\_C\_KS\_20130927.fits \\
P161-D & C & KS & 2013-10-15 & 56580 & -- & P161-D\_C\_KS\_20131015.fits \\
P161-D & C & KS & 2013-10-20 & 56585 & -- & P161-D\_C\_KS\_20131020.fits \\
P212-C & A & H & 2013-04-25 & 56407 & -- & P212-C\_A\_H\_20130425.fits \\
P212-C & A & H & 2013-04-29 & 56411 & -- & P212-C\_A\_H\_20130429.fits \\
P212-C & A & H & 2013-05-19 & 56431 & -- & P212-C\_A\_H\_20130519.fits \\
P212-C & A & J & 2013-03-26 & 56377 & -- & P212-C\_A\_J\_20130326.fits \\
P212-C & A & J & 2013-04-20 & 56402 & -- & P212-C\_A\_J\_20130420.fits \\
P212-C & A & J & 2013-04-29 & 56411 & -- & P212-C\_A\_J\_20130429.fits \\
P212-C & A & J & 2013-05-19 & 56431 & -- & P212-C\_A\_J\_20130519.fits \\
P212-C & A & KS & 2013-03-26 & 56377 & -- & P212-C\_A\_KS\_20130326.fits \\
P212-C & A & KS & 2013-04-20 & 56402 & -- & P212-C\_A\_KS\_20130420.fits \\
P212-C & B & H & 2013-04-20 & 56402 & -- & P212-C\_B\_H\_20130420.fits \\
P212-C & B & H & 2013-04-25 & 56407 & -- & P212-C\_B\_H\_20130425.fits \\
P212-C & B & H & 2013-04-29 & 56411 & -- & P212-C\_B\_H\_20130429.fits \\
P212-C & B & J & 2013-04-20 & 56402 & -- & P212-C\_B\_J\_20130420.fits \\
P212-C & B & J & 2013-04-25 & 56407 & -- & P212-C\_B\_J\_20130425.fits \\
P212-C & B & J & 2013-04-29 & 56411 & -- & P212-C\_B\_J\_20130429.fits \\
P212-C & B & KS & 2013-04-20 & 56402 & -- & P212-C\_B\_KS\_20130420.fits \\
P212-C & B & KS & 2013-04-25 & 56407 & -- & P212-C\_B\_KS\_20130425.fits \\
P212-C & B & KS & 2013-04-29 & 56411 & -- & P212-C\_B\_KS\_20130429.fits \\
P212-C & C & H & 2013-04-20 & 56402 & -- & P212-C\_C\_H\_20130420.fits \\
P212-C & C & J & 2013-04-20 & 56402 & -- & P212-C\_C\_J\_20130420.fits \\
P212-C & C & KS & 2013-04-20 & 56402 & -- & P212-C\_C\_KS\_20130420.fits \\
P330-E & A & H & 2013-05-19 & 56431 & -- & P330-E\_A\_H\_20130519.fits \\
P330-E & A & H & 2013-05-22 & 56434 & -- & P330-E\_A\_H\_20130522.fits \\
P330-E & A & H & 2013-05-23 & 56435 & -- & P330-E\_A\_H\_20130523.fits \\
P330-E & A & H & 2013-05-28 & 56440 & -- & P330-E\_A\_H\_20130528.fits \\
P330-E & A & H & 2013-06-13 & 56456 & -- & P330-E\_A\_H\_20130613.fits \\
P330-E & A & J & 2013-05-19 & 56431 & -- & P330-E\_A\_J\_20130519.fits \\
P330-E & A & J & 2013-05-22 & 56434 & -- & P330-E\_A\_J\_20130522.fits \\
P330-E & A & J & 2013-05-23 & 56435 & -- & P330-E\_A\_J\_20130523.fits \\
P330-E & A & J & 2013-05-28 & 56440 & -- & P330-E\_A\_J\_20130528.fits \\
P330-E & A & J & 2013-06-13 & 56456 & -- & P330-E\_A\_J\_20130613.fits \\
P330-E & A & KS & 2013-05-19 & 56431 & -- & P330-E\_A\_KS\_20130519.fits \\
P330-E & A & KS & 2013-05-22 & 56434 & -- & P330-E\_A\_KS\_20130522.fits \\
P330-E & A & KS & 2013-05-23 & 56435 & -- & P330-E\_A\_KS\_20130523.fits \\
P330-E & A & KS & 2013-05-28 & 56440 & -- & P330-E\_A\_KS\_20130528.fits \\
P330-E & A & KS & 2013-06-13 & 56456 & -- & P330-E\_A\_KS\_20130613.fits \\
P330-E & B & H & 2013-05-22 & 56434 & -- & P330-E\_B\_H\_20130522.fits \\
P330-E & B & H & 2013-05-28 & 56440 & -- & P330-E\_B\_H\_20130528.fits \\
P330-E & B & H & 2013-06-17 & 56460 & -- & P330-E\_B\_H\_20130617.fits \\
P330-E & B & J & 2013-05-22 & 56434 & -- & P330-E\_B\_J\_20130522.fits \\
P330-E & B & J & 2013-05-28 & 56440 & -- & P330-E\_B\_J\_20130528.fits \\
P330-E & B & J & 2013-06-17 & 56460 & -- & P330-E\_B\_J\_20130617.fits \\
P330-E & B & KS & 2013-05-22 & 56434 & -- & P330-E\_B\_KS\_20130522.fits \\
P330-E & B & KS & 2013-05-28 & 56440 & -- & P330-E\_B\_KS\_20130528.fits \\
P330-E & B & KS & 2013-06-17 & 56460 & -- & P330-E\_B\_KS\_20130617.fits \\
P525-E & A & H & 2012-11-22 & 56253 & -- & P525-E\_A\_H\_20121122.fits \\
P525-E & A & H & 2012-11-25 & 56256 & -- & P525-E\_A\_H\_20121125.fits \\
P525-E & A & H & 2012-11-30 & 56261 & -- & P525-E\_A\_H\_20121130.fits \\
P525-E & A & H & 2013-09-25 & 56560 & -- & P525-E\_A\_H\_20130925.fits \\
P525-E & A & H & 2013-09-27 & 56562 & -- & P525-E\_A\_H\_20130927.fits \\
P525-E & A & H & 2013-10-15 & 56580 & -- & P525-E\_A\_H\_20131015.fits \\
P525-E & A & H & 2013-10-19 & 56584 & -- & P525-E\_A\_H\_20131019.fits \\
P525-E & A & H & 2013-10-20 & 56585 & -- & P525-E\_A\_H\_20131020.fits \\
P525-E & A & H & 2013-11-11 & 56607 & -- & P525-E\_A\_H\_20131111.fits \\
P525-E & A & H & 2013-11-20 & 56616 & -- & P525-E\_A\_H\_20131120.fits \\
P525-E & A & H & 2013-12-09 & 56635 & -- & P525-E\_A\_H\_20131209.fits \\
P525-E & A & H & 2013-12-13 & 56639 & -- & P525-E\_A\_H\_20131213.fits \\
P525-E & A & J & 2012-11-22 & 56253 & -- & P525-E\_A\_J\_20121122.fits \\
P525-E & A & J & 2012-11-25 & 56256 & -- & P525-E\_A\_J\_20121125.fits \\
P525-E & A & J & 2012-11-30 & 56261 & -- & P525-E\_A\_J\_20121130.fits \\
P525-E & A & J & 2013-09-27 & 56562 & -- & P525-E\_A\_J\_20130927.fits \\
P525-E & A & J & 2013-10-15 & 56580 & -- & P525-E\_A\_J\_20131015.fits \\
P525-E & A & J & 2013-11-11 & 56607 & -- & P525-E\_A\_J\_20131111.fits \\
P525-E & A & J & 2013-12-09 & 56635 & -- & P525-E\_A\_J\_20131209.fits \\
P525-E & A & KS & 2012-11-22 & 56253 & -- & P525-E\_A\_KS\_20121122.fits \\
P525-E & A & KS & 2012-11-25 & 56256 & -- & P525-E\_A\_KS\_20121125.fits \\
P525-E & A & KS & 2012-11-30 & 56261 & -- & P525-E\_A\_KS\_20121130.fits \\
P525-E & A & KS & 2013-09-27 & 56562 & -- & P525-E\_A\_KS\_20130927.fits \\
P525-E & A & KS & 2013-10-15 & 56580 & -- & P525-E\_A\_KS\_20131015.fits \\
P525-E & A & KS & 2013-11-11 & 56607 & -- & P525-E\_A\_KS\_20131111.fits \\
P525-E & A & KS & 2013-12-09 & 56635 & -- & P525-E\_A\_KS\_20131209.fits \\
P525-E & A & KS & 2013-12-13 & 56639 & -- & P525-E\_A\_KS\_20131213.fits \\
P525-E & B & H & 2012-11-22 & 56253 & -- & P525-E\_B\_H\_20121122.fits \\
P525-E & B & H & 2012-11-25 & 56256 & -- & P525-E\_B\_H\_20121125.fits \\
P525-E & B & H & 2012-11-30 & 56261 & -- & P525-E\_B\_H\_20121130.fits \\
P525-E & B & H & 2013-09-27 & 56562 & -- & P525-E\_B\_H\_20130927.fits \\
P525-E & B & H & 2013-10-15 & 56580 & -- & P525-E\_B\_H\_20131015.fits \\
P525-E & B & H & 2013-10-19 & 56584 & -- & P525-E\_B\_H\_20131019.fits \\
P525-E & B & H & 2013-10-20 & 56585 & -- & P525-E\_B\_H\_20131020.fits \\
P525-E & B & H & 2013-11-11 & 56607 & -- & P525-E\_B\_H\_20131111.fits \\
P525-E & B & H & 2013-12-09 & 56635 & -- & P525-E\_B\_H\_20131209.fits \\
P525-E & B & H & 2013-12-13 & 56639 & -- & P525-E\_B\_H\_20131213.fits \\
P525-E & B & J & 2012-11-22 & 56253 & -- & P525-E\_B\_J\_20121122.fits \\
P525-E & B & J & 2012-11-25 & 56256 & -- & P525-E\_B\_J\_20121125.fits \\
P525-E & B & J & 2012-11-30 & 56261 & -- & P525-E\_B\_J\_20121130.fits \\
P525-E & B & J & 2013-09-27 & 56562 & -- & P525-E\_B\_J\_20130927.fits \\
P525-E & B & J & 2013-10-15 & 56580 & -- & P525-E\_B\_J\_20131015.fits \\
P525-E & B & J & 2013-10-19 & 56584 & -- & P525-E\_B\_J\_20131019.fits \\
P525-E & B & J & 2013-10-20 & 56585 & -- & P525-E\_B\_J\_20131020.fits \\
P525-E & B & J & 2013-11-11 & 56607 & -- & P525-E\_B\_J\_20131111.fits \\
P525-E & B & J & 2013-12-09 & 56635 & -- & P525-E\_B\_J\_20131209.fits \\
P525-E & B & J & 2013-12-13 & 56639 & -- & P525-E\_B\_J\_20131213.fits \\
P525-E & B & KS & 2012-11-22 & 56253 & -- & P525-E\_B\_KS\_20121122.fits \\
P525-E & B & KS & 2012-11-25 & 56256 & -- & P525-E\_B\_KS\_20121125.fits \\
P525-E & B & KS & 2012-11-30 & 56261 & -- & P525-E\_B\_KS\_20121130.fits \\
P525-E & B & KS & 2013-09-27 & 56562 & -- & P525-E\_B\_KS\_20130927.fits \\
P525-E & B & KS & 2013-10-15 & 56580 & -- & P525-E\_B\_KS\_20131015.fits \\
P525-E & B & KS & 2013-10-19 & 56584 & -- & P525-E\_B\_KS\_20131019.fits \\
P525-E & B & KS & 2013-10-20 & 56585 & -- & P525-E\_B\_KS\_20131020.fits \\
P525-E & B & KS & 2013-11-11 & 56607 & -- & P525-E\_B\_KS\_20131111.fits \\
P525-E & B & KS & 2013-12-09 & 56635 & -- & P525-E\_B\_KS\_20131209.fits \\
P525-E & B & KS & 2013-12-13 & 56639 & -- & P525-E\_B\_KS\_20131213.fits \\
P525-E & C & H & 2012-11-25 & 56256 & -- & P525-E\_C\_H\_20121125.fits \\
P525-E & C & H & 2013-09-27 & 56562 & -- & P525-E\_C\_H\_20130927.fits \\
P525-E & C & H & 2013-10-15 & 56580 & -- & P525-E\_C\_H\_20131015.fits \\
P525-E & C & H & 2013-10-19 & 56584 & -- & P525-E\_C\_H\_20131019.fits \\
P525-E & C & H & 2013-10-20 & 56585 & -- & P525-E\_C\_H\_20131020.fits \\
P525-E & C & H & 2013-11-11 & 56607 & -- & P525-E\_C\_H\_20131111.fits \\
P525-E & C & J & 2012-11-25 & 56256 & -- & P525-E\_C\_J\_20121125.fits \\
P525-E & C & J & 2013-09-27 & 56562 & -- & P525-E\_C\_J\_20130927.fits \\
P525-E & C & J & 2013-10-15 & 56580 & -- & P525-E\_C\_J\_20131015.fits \\
P525-E & C & J & 2013-10-19 & 56584 & -- & P525-E\_C\_J\_20131019.fits \\
P525-E & C & J & 2013-10-20 & 56585 & -- & P525-E\_C\_J\_20131020.fits \\
P525-E & C & J & 2013-11-11 & 56607 & -- & P525-E\_C\_J\_20131111.fits \\
P525-E & C & KS & 2012-11-25 & 56256 & -- & P525-E\_C\_KS\_20121125.fits \\
P525-E & C & KS & 2013-09-27 & 56562 & -- & P525-E\_C\_KS\_20130927.fits \\
P525-E & C & KS & 2013-10-15 & 56580 & -- & P525-E\_C\_KS\_20131015.fits \\
P525-E & C & KS & 2013-10-19 & 56584 & -- & P525-E\_C\_KS\_20131019.fits \\
P525-E & C & KS & 2013-10-20 & 56585 & -- & P525-E\_C\_KS\_20131020.fits \\
P525-E & C & KS & 2013-11-11 & 56607 & -- & P525-E\_C\_KS\_20131111.fits \\
PS1-12bwh & A & H & 2012-10-28 & 56228 & 6 & PS1-12bwh\_A\_H\_20121028.fits \\
PS1-12bwh & A & H & 2012-11-02 & 56233 & 11 & PS1-12bwh\_A\_H\_20121102.fits \\
PS1-12bwh & A & H & 2012-11-22 & 56253 & 31 & PS1-12bwh\_A\_H\_20121122.fits \\
PS1-12bwh & A & H & 2012-11-25 & 56256 & 34 & PS1-12bwh\_A\_H\_20121125.fits \\
PS1-12bwh & A & H & 2012-11-30 & 56261 & 39 & PS1-12bwh\_A\_H\_20121130.fits \\
PS1-12bwh & A & J & 2012-10-28 & 56228 & 6 & PS1-12bwh\_A\_J\_20121028.fits \\
PS1-12bwh & A & J & 2012-11-02 & 56233 & 11 & PS1-12bwh\_A\_J\_20121102.fits \\
PS1-12bwh & A & J & 2012-11-22 & 56253 & 31 & PS1-12bwh\_A\_J\_20121122.fits \\
PS1-12bwh & A & J & 2012-11-25 & 56256 & 34 & PS1-12bwh\_A\_J\_20121125.fits \\
PS1-12bwh & A & J & 2012-11-30 & 56261 & 39 & PS1-12bwh\_A\_J\_20121130.fits \\
PS1-13dkh & A & H & 2013-10-18 & 56583 & 11 & PS1-13dkh\_A\_H\_20131018.fits \\
PS1-13dkh & A & H & 2013-11-11 & 56607 & 35 & PS1-13dkh\_A\_H\_20131111.fits \\
PS1-13dkh & A & H & 2013-11-20 & 56616 & 44 & PS1-13dkh\_A\_H\_20131120.fits \\
PS1-13dkh & A & H & 2013-12-09 & 56635 & 63 & PS1-13dkh\_A\_H\_20131209.fits \\
PS1-13dkh & A & J & 2013-10-18 & 56583 & 11 & PS1-13dkh\_A\_J\_20131018.fits \\
PS1-13dkh & A & J & 2013-11-11 & 56607 & 35 & PS1-13dkh\_A\_J\_20131111.fits \\
PS1-13dkh & A & J & 2013-11-20 & 56616 & 44 & PS1-13dkh\_A\_J\_20131120.fits \\
PS1-13dkh & A & J & 2013-12-09 & 56635 & 63 & PS1-13dkh\_A\_J\_20131209.fits \\
PSNJ07250042+2347030 & A & H & 2012-10-28 & 56228 & 10 & PSNJ07250042+2347030\_A\_H\_20121028.fits \\
PSNJ07250042+2347030 & A & H & 2012-11-02 & 56233 & 15 & PSNJ07250042+2347030\_A\_H\_20121102.fits \\
PSNJ07250042+2347030 & A & H & 2012-11-22 & 56253 & 35 & PSNJ07250042+2347030\_A\_H\_20121122.fits \\
PSNJ07250042+2347030 & A & H & 2012-11-25 & 56256 & 38 & PSNJ07250042+2347030\_A\_H\_20121125.fits \\
PSNJ07250042+2347030 & A & H & 2012-11-30 & 56261 & 43 & PSNJ07250042+2347030\_A\_H\_20121130.fits \\
PSNJ07250042+2347030 & A & H & 2013-12-13 & 56639 & 421 & PSNJ07250042+2347030\_A\_H\_20131213.fits \\
PSNJ07250042+2347030 & A & J & 2012-10-28 & 56228 & 10 & PSNJ07250042+2347030\_A\_J\_20121028.fits \\
PSNJ07250042+2347030 & A & J & 2012-11-02 & 56233 & 15 & PSNJ07250042+2347030\_A\_J\_20121102.fits \\
PSNJ07250042+2347030 & A & J & 2012-11-22 & 56253 & 35 & PSNJ07250042+2347030\_A\_J\_20121122.fits \\
PSNJ07250042+2347030 & A & J & 2012-11-25 & 56256 & 38 & PSNJ07250042+2347030\_A\_J\_20121125.fits \\
PSNJ07250042+2347030 & A & J & 2012-11-30 & 56261 & 43 & PSNJ07250042+2347030\_A\_J\_20121130.fits \\
PSNJ07250042+2347030 & A & J & 2013-12-13 & 56639 & 421 & PSNJ07250042+2347030\_A\_J\_20131213.fits \\
PTF11moy & A & H & 2011-10-25 & 55859 & 35 & PTF11moy\_A\_H\_20111025.fits \\
PTF11moy & A & J & 2011-10-25 & 55859 & 35 & PTF11moy\_A\_J\_20111025.fits \\
PTF11mty & A & H & 2011-10-25 & 55859 & 24 & PTF11mty\_A\_H\_20111025.fits \\
PTF11mty & A & H & 2011-11-15 & 55880 & 45 & PTF11mty\_A\_H\_20111115.fits \\
PTF11mty & A & H & 2012-09-25 & 56195 & 360 & PTF11mty\_A\_H\_20120925.fits \\
PTF11mty & A & J & 2011-10-25 & 55859 & 24 & PTF11mty\_A\_J\_20111025.fits \\
PTF11mty & A & J & 2011-11-15 & 55880 & 45 & PTF11mty\_A\_J\_20111115.fits \\
PTF11mty & A & J & 2012-10-07 & 56207 & 372 & PTF11mty\_A\_J\_20121007.fits \\
PTF11owc & A & H & 2011-11-15 & 55880 & 13 & PTF11owc\_A\_H\_20111115.fits \\
PTF11owc & A & H & 2011-11-21 & 55886 & 19 & PTF11owc\_A\_H\_20111121.fits \\
PTF11owc & A & H & 2011-12-08 & 55903 & 36 & PTF11owc\_A\_H\_20111208.fits \\
PTF11owc & A & H & 2012-04-02 & 56019 & 152 & PTF11owc\_A\_H\_20120402.fits \\
PTF11owc & A & H & 2012-11-25 & 56256 & 389 & PTF11owc\_A\_H\_20121125.fits \\
PTF11owc & A & J & 2011-11-15 & 55880 & 13 & PTF11owc\_A\_J\_20111115.fits \\
PTF11owc & A & J & 2011-11-21 & 55886 & 19 & PTF11owc\_A\_J\_20111121.fits \\
PTF11owc & A & J & 2011-12-08 & 55903 & 36 & PTF11owc\_A\_J\_20111208.fits \\
PTF11owc & A & J & 2012-04-02 & 56019 & 152 & PTF11owc\_A\_J\_20120402.fits \\
PTF11qmo & A & H & 2011-12-08 & 55903 & 9 & PTF11qmo\_A\_H\_20111208.fits \\
PTF11qmo & A & H & 2012-01-08 & 55934 & 40 & PTF11qmo\_A\_H\_20120108.fits \\
PTF11qmo & A & J & 2011-12-08 & 55903 & 9 & PTF11qmo\_A\_J\_20111208.fits \\
PTF11qmo & A & J & 2012-01-08 & 55934 & 40 & PTF11qmo\_A\_J\_20120108.fits \\
PTF11qpc & A & H & 2011-12-08 & 55903 & 1 & PTF11qpc\_A\_H\_20111208.fits \\
PTF11qpc & A & H & 2012-01-08 & 55934 & 32 & PTF11qpc\_A\_H\_20120108.fits \\
PTF11qpc & A & H & 2012-04-02 & 56019 & 117 & PTF11qpc\_A\_H\_20120402.fits \\
PTF11qri & A & H & 2011-12-08 & 55903 & 6 & PTF11qri\_A\_H\_20111208.fits \\
PTF11qri & A & H & 2012-01-08 & 55934 & 37 & PTF11qri\_A\_H\_20120108.fits \\
PTF11qri & A & J & 2011-12-08 & 55903 & 6 & PTF11qri\_A\_J\_20111208.fits \\
PTF11qri & A & J & 2012-01-08 & 55934 & 37 & PTF11qri\_A\_J\_20120108.fits \\
PTF11qzq & A & H & 2011-12-08 & 55903 & -2 & PTF11qzq\_A\_H\_20111208.fits \\
PTF11qzq & A & H & 2012-01-08 & 55934 & 29 & PTF11qzq\_A\_H\_20120108.fits \\
PTF11qzq & A & H & 2012-10-07 & 56207 & 302 & PTF11qzq\_A\_H\_20121007.fits \\
PTF11qzq & A & J & 2011-12-08 & 55903 & -2 & PTF11qzq\_A\_J\_20111208.fits \\
PTF11qzq & A & J & 2012-01-08 & 55934 & 29 & PTF11qzq\_A\_J\_20120108.fits \\
PTF11qzq & A & J & 2013-09-25 & 56560 & 655 & PTF11qzq\_A\_J\_20130925.fits \\
PTF12iiq & A & H & 2012-09-25 & 56195 & 16 & PTF12iiq\_A\_H\_20120925.fits \\
PTF12iiq & A & H & 2012-10-01 & 56201 & 22 & PTF12iiq\_A\_H\_20121001.fits \\
PTF12iiq & A & H & 2012-10-07 & 56207 & 28 & PTF12iiq\_A\_H\_20121007.fits \\
PTF12iiq & A & J & 2012-09-25 & 56195 & 16 & PTF12iiq\_A\_J\_20120925.fits \\
PTF12iiq & A & J & 2012-10-01 & 56201 & 22 & PTF12iiq\_A\_J\_20121001.fits \\
PTF12iiq & A & J & 2012-10-07 & 56207 & 28 & PTF12iiq\_A\_J\_20121007.fits \\
PTF12ikt & A & H & 2012-09-25 & 56195 & 13 & PTF12ikt\_A\_H\_20120925.fits \\
PTF12ikt & A & H & 2012-10-01 & 56201 & 19 & PTF12ikt\_A\_H\_20121001.fits \\
PTF12ikt & A & H & 2012-10-07 & 56207 & 25 & PTF12ikt\_A\_H\_20121007.fits \\
PTF12ikt & A & J & 2012-09-25 & 56195 & 13 & PTF12ikt\_A\_J\_20120925.fits \\
PTF12ikt & A & J & 2012-10-01 & 56201 & 19 & PTF12ikt\_A\_J\_20121001.fits \\
PTF12ikt & A & J & 2012-10-07 & 56207 & 25 & PTF12ikt\_A\_J\_20121007.fits \\
PTF13asv & A & H & 2013-05-22 & 56434 & 11 & PTF13asv\_A\_H\_20130522.fits \\
PTF13asv & A & H & 2013-05-28 & 56440 & 17 & PTF13asv\_A\_H\_20130528.fits \\
PTF13asv & A & H & 2013-06-13 & 56456 & 33 & PTF13asv\_A\_H\_20130613.fits \\
PTF13asv & A & H & 2013-06-17 & 56460 & 37 & PTF13asv\_A\_H\_20130617.fits \\
PTF13asv & A & J & 2013-05-22 & 56434 & 11 & PTF13asv\_A\_J\_20130522.fits \\
PTF13asv & A & J & 2013-05-28 & 56440 & 17 & PTF13asv\_A\_J\_20130528.fits \\
PTF13asv & A & J & 2013-06-13 & 56456 & 33 & PTF13asv\_A\_J\_20130613.fits \\
PTF13asv & A & J & 2013-06-17 & 56460 & 37 & PTF13asv\_A\_J\_20130617.fits \\
PTF13ayw & A & H & 2013-05-19 & 56431 & 1 & PTF13ayw\_A\_H\_20130519.fits \\
PTF13ayw & A & H & 2013-05-28 & 56440 & 10 & PTF13ayw\_A\_H\_20130528.fits \\
PTF13ayw & A & H & 2013-06-13 & 56456 & 26 & PTF13ayw\_A\_H\_20130613.fits \\
PTF13ayw & A & H & 2013-06-17 & 56460 & 30 & PTF13ayw\_A\_H\_20130617.fits \\
PTF13ayw & A & J & 2013-05-19 & 56431 & 1 & PTF13ayw\_A\_J\_20130519.fits \\
PTF13ayw & A & J & 2013-05-28 & 56440 & 10 & PTF13ayw\_A\_J\_20130528.fits \\
PTF13ayw & A & J & 2013-06-13 & 56456 & 26 & PTF13ayw\_A\_J\_20130613.fits \\
PTF13ayw & A & J & 2013-06-17 & 56460 & 30 & PTF13ayw\_A\_J\_20130617.fits \\
PTF13dad & A & H & 2013-09-25 & 56560 & 13 & PTF13dad\_A\_H\_20130925.fits \\
PTF13dad & A & H & 2013-10-15 & 56580 & 33 & PTF13dad\_A\_H\_20131015.fits \\
PTF13dad & A & H & 2013-10-20 & 56585 & 38 & PTF13dad\_A\_H\_20131020.fits \\
PTF13dad & A & J & 2013-09-25 & 56560 & 13 & PTF13dad\_A\_J\_20130925.fits \\
PTF13dad & A & J & 2013-10-15 & 56580 & 33 & PTF13dad\_A\_J\_20131015.fits \\
PTF13dad & A & J & 2013-10-20 & 56585 & 38 & PTF13dad\_A\_J\_20131020.fits \\
PTF13ddg & A & H & 2013-09-25 & 56560 & 15 & PTF13ddg\_A\_H\_20130925.fits \\
PTF13ddg & A & H & 2013-10-15 & 56580 & 35 & PTF13ddg\_A\_H\_20131015.fits \\
PTF13ddg & A & H & 2013-10-19 & 56584 & 39 & PTF13ddg\_A\_H\_20131019.fits \\
S791-C & A & H & 2013-05-23 & 56435 & -- & S791-C\_A\_H\_20130523.fits \\
S791-C & A & H & 2013-05-28 & 56440 & -- & S791-C\_A\_H\_20130528.fits \\
S791-C & A & H & 2013-06-13 & 56456 & -- & S791-C\_A\_H\_20130613.fits \\
S791-C & A & H & 2013-06-17 & 56460 & -- & S791-C\_A\_H\_20130617.fits \\
S791-C & A & J & 2013-05-23 & 56435 & -- & S791-C\_A\_J\_20130523.fits \\
S791-C & A & J & 2013-05-28 & 56440 & -- & S791-C\_A\_J\_20130528.fits \\
S791-C & A & J & 2013-06-13 & 56456 & -- & S791-C\_A\_J\_20130613.fits \\
S791-C & A & J & 2013-06-17 & 56460 & -- & S791-C\_A\_J\_20130617.fits \\
S791-C & A & KS & 2013-05-23 & 56435 & -- & S791-C\_A\_KS\_20130523.fits \\
S791-C & A & KS & 2013-05-28 & 56440 & -- & S791-C\_A\_KS\_20130528.fits \\
S791-C & A & KS & 2013-06-13 & 56456 & -- & S791-C\_A\_KS\_20130613.fits \\
S791-C & A & KS & 2013-06-17 & 56460 & -- & S791-C\_A\_KS\_20130617.fits \\
S791-C & B & H & 2013-05-23 & 56435 & -- & S791-C\_B\_H\_20130523.fits \\
S791-C & B & H & 2013-05-28 & 56440 & -- & S791-C\_B\_H\_20130528.fits \\
S791-C & B & J & 2013-05-23 & 56435 & -- & S791-C\_B\_J\_20130523.fits \\
S791-C & B & J & 2013-05-28 & 56440 & -- & S791-C\_B\_J\_20130528.fits \\
S791-C & B & KS & 2013-05-23 & 56435 & -- & S791-C\_B\_KS\_20130523.fits \\
S791-C & B & KS & 2013-05-28 & 56440 & -- & S791-C\_B\_KS\_20130528.fits \\
S840-F & A & H & 2013-10-15 & 56580 & -- & S840-F\_A\_H\_20131015.fits \\
S840-F & A & J & 2013-10-15 & 56580 & -- & S840-F\_A\_J\_20131015.fits \\
S840-F & A & KS & 2013-10-15 & 56580 & -- & S840-F\_A\_KS\_20131015.fits \\
SN2011fe & A & H & 2011-10-25 & 55859 & 45 & SN2011fe\_A\_H\_20111025.fits \\
SN2011fe & A & H & 2012-04-02 & 56019 & 205 & SN2011fe\_A\_H\_20120402.fits \\
SN2011fe & A & J & 2011-10-25 & 55859 & 45 & SN2011fe\_A\_J\_20111025.fits \\
SN2011fe & A & J & 2012-04-02 & 56019 & 205 & SN2011fe\_A\_J\_20120402.fits \\
SN2011fe & A & KS & 2011-10-25 & 55859 & 45 & SN2011fe\_A\_KS\_20111025.fits \\
SN2011fs & A & H & 2011-10-25 & 55859 & 26 & SN2011fs\_A\_H\_20111025.fits \\
SN2011fs & A & H & 2011-11-15 & 55880 & 47 & SN2011fs\_A\_H\_20111115.fits \\
SN2011fs & A & H & 2011-12-08 & 55903 & 70 & SN2011fs\_A\_H\_20111208.fits \\
SN2011fs & A & H & 2012-01-08 & 55934 & 101 & SN2011fs\_A\_H\_20120108.fits \\
SN2011fs & A & J & 2011-10-25 & 55859 & 26 & SN2011fs\_A\_J\_20111025.fits \\
SN2011fs & A & J & 2011-11-15 & 55880 & 47 & SN2011fs\_A\_J\_20111115.fits \\
SN2011fs & A & J & 2011-12-08 & 55903 & 70 & SN2011fs\_A\_J\_20111208.fits \\
SN2011fs & A & J & 2012-01-08 & 55934 & 101 & SN2011fs\_A\_J\_20120108.fits \\
SN2011fs & A & KS & 2011-10-25 & 55859 & 26 & SN2011fs\_A\_KS\_20111025.fits \\
SN2011gf & A & H & 2011-10-25 & 55859 & 32 & SN2011gf\_A\_H\_20111025.fits \\
SN2011gf & A & H & 2011-11-15 & 55880 & 53 & SN2011gf\_A\_H\_20111115.fits \\
SN2011gf & A & H & 2011-12-08 & 55903 & 76 & SN2011gf\_A\_H\_20111208.fits \\
SN2011gf & A & J & 2011-10-25 & 55859 & 32 & SN2011gf\_A\_J\_20111025.fits \\
SN2011gf & A & J & 2011-11-15 & 55880 & 53 & SN2011gf\_A\_J\_20111115.fits \\
SN2011gy & A & H & 2011-11-15 & 55880 & 15 & SN2011gy\_A\_H\_20111115.fits \\
SN2011gy & A & H & 2011-11-21 & 55886 & 21 & SN2011gy\_A\_H\_20111121.fits \\
SN2011gy & A & H & 2011-12-08 & 55903 & 38 & SN2011gy\_A\_H\_20111208.fits \\
SN2011gy & A & H & 2012-01-08 & 55934 & 69 & SN2011gy\_A\_H\_20120108.fits \\
SN2011gy & A & H & 2012-04-02 & 56019 & 154 & SN2011gy\_A\_H\_20120402.fits \\
SN2011gy & A & H & 2012-10-28 & 56228 & 363 & SN2011gy\_A\_H\_20121028.fits \\
SN2011gy & A & J & 2011-11-15 & 55880 & 15 & SN2011gy\_A\_J\_20111115.fits \\
SN2011gy & A & J & 2011-11-21 & 55886 & 21 & SN2011gy\_A\_J\_20111121.fits \\
SN2011gy & A & J & 2011-12-08 & 55903 & 38 & SN2011gy\_A\_J\_20111208.fits \\
SN2011gy & A & J & 2012-01-08 & 55934 & 69 & SN2011gy\_A\_J\_20120108.fits \\
SN2011gy & A & J & 2012-10-28 & 56228 & 363 & SN2011gy\_A\_J\_20121028.fits \\
SN2011ha & A & H & 2011-11-15 & 55880 & 40 & SN2011ha\_A\_H\_20111115.fits \\
SN2011ha & A & H & 2011-11-21 & 55886 & 46 & SN2011ha\_A\_H\_20111121.fits \\
SN2011ha & A & J & 2011-11-15 & 55880 & 40 & SN2011ha\_A\_J\_20111115.fits \\
SN2011hb & A & H & 2011-11-15 & 55880 & 8 & SN2011hb\_A\_H\_20111115.fits \\
SN2011hb & A & H & 2011-12-08 & 55903 & 31 & SN2011hb\_A\_H\_20111208.fits \\
SN2011hb & A & H & 2012-01-08 & 55934 & 62 & SN2011hb\_A\_H\_20120108.fits \\
SN2011hb & A & H & 2013-10-20 & 56585 & 713 & SN2011hb\_A\_H\_20131020.fits \\
SN2011hb & A & J & 2011-11-15 & 55880 & 8 & SN2011hb\_A\_J\_20111115.fits \\
SN2011hb & A & J & 2011-12-08 & 55903 & 31 & SN2011hb\_A\_J\_20111208.fits \\
SN2011hb & A & J & 2012-01-08 & 55934 & 62 & SN2011hb\_A\_J\_20120108.fits \\
SN2011hb & A & J & 2013-10-20 & 56585 & 713 & SN2011hb\_A\_J\_20131020.fits \\
SN2011hk & A & H & 2011-11-15 & 55880 & 16 & SN2011hk\_A\_H\_20111115.fits \\
SN2011hk & A & H & 2011-12-08 & 55903 & 39 & SN2011hk\_A\_H\_20111208.fits \\
SN2011hk & A & H & 2012-01-08 & 55934 & 70 & SN2011hk\_A\_H\_20120108.fits \\
SN2011hk & A & J & 2011-11-15 & 55880 & 16 & SN2011hk\_A\_J\_20111115.fits \\
SN2011hk & A & J & 2011-12-08 & 55903 & 39 & SN2011hk\_A\_J\_20111208.fits \\
SN2011hk & A & J & 2012-01-08 & 55934 & 70 & SN2011hk\_A\_J\_20120108.fits \\
SN2011ho & A & H & 2011-11-21 & 55886 & 21 & SN2011ho\_A\_H\_20111121.fits \\
SN2011ho & A & H & 2011-12-08 & 55903 & 38 & SN2011ho\_A\_H\_20111208.fits \\
SN2011ho & A & H & 2012-01-08 & 55934 & 69 & SN2011ho\_A\_H\_20120108.fits \\
SN2011ho & A & H & 2012-04-02 & 56019 & 154 & SN2011ho\_A\_H\_20120402.fits \\
SN2011hr & A & H & 2011-11-21 & 55886 & 3 & SN2011hr\_A\_H\_20111121.fits \\
SN2011hr & A & H & 2011-12-08 & 55903 & 20 & SN2011hr\_A\_H\_20111208.fits \\
SN2011hr & A & H & 2012-01-08 & 55934 & 51 & SN2011hr\_A\_H\_20120108.fits \\
SN2011hr & A & H & 2012-04-02 & 56019 & 136 & SN2011hr\_A\_H\_20120402.fits \\
SN2011hr & A & H & 2013-12-13 & 56639 & 756 & SN2011hr\_A\_H\_20131213.fits \\
SN2011hr & A & J & 2011-11-21 & 55886 & 3 & SN2011hr\_A\_J\_20111121.fits \\
SN2011hr & A & J & 2011-12-08 & 55903 & 20 & SN2011hr\_A\_J\_20111208.fits \\
SN2011hr & A & J & 2012-01-08 & 55934 & 51 & SN2011hr\_A\_J\_20120108.fits \\
SN2011hr & A & J & 2012-04-02 & 56019 & 136 & SN2011hr\_A\_J\_20120402.fits \\
SN2011io & A & H & 2011-12-08 & 55903 & 9 & SN2011io\_A\_H\_20111208.fits \\
SN2011io & A & J & 2011-12-08 & 55903 & 9 & SN2011io\_A\_J\_20111208.fits \\
SN2011iu & A & H & 2011-12-08 & 55903 & 9 & SN2011iu\_A\_H\_20111208.fits \\
SN2011iu & A & H & 2012-01-08 & 55934 & 40 & SN2011iu\_A\_H\_20120108.fits \\
SN2011iu & A & H & 2012-09-25 & 56195 & 301 & SN2011iu\_A\_H\_20120925.fits \\
SN2011iu & A & J & 2011-12-08 & 55903 & 9 & SN2011iu\_A\_J\_20111208.fits \\
SN2011iu & A & J & 2012-01-08 & 55934 & 40 & SN2011iu\_A\_J\_20120108.fits \\
SN2011iu & A & J & 2012-10-01 & 56201 & 307 & SN2011iu\_A\_J\_20121001.fits \\
SN2011iy & A & H & 2012-04-02 & 56019 & 123 & SN2011iy\_A\_H\_20120402.fits \\
SN2011iy & A & J & 2012-04-02 & 56019 & 123 & SN2011iy\_A\_J\_20120402.fits \\
SN2011jh & A & H & 2012-04-02 & 56019 & 90 & SN2011jh\_A\_H\_20120402.fits \\
SN2011jh & A & J & 2012-04-02 & 56019 & 90 & SN2011jh\_A\_J\_20120402.fits \\
SN2012bh & A & H & 2012-04-02 & 56019 & 3 & SN2012bh\_A\_H\_20120402.fits \\
SN2012bh & A & J & 2012-04-02 & 56019 & 3 & SN2012bh\_A\_J\_20120402.fits \\
SN2012bm & A & H & 2012-04-02 & 56019 & -2 & SN2012bm\_A\_H\_20120402.fits \\
SN2012bm & A & J & 2012-04-02 & 56019 & -2 & SN2012bm\_A\_J\_20120402.fits \\
SN2012bo & A & H & 2012-04-02 & 56019 & -2 & SN2012bo\_A\_H\_20120402.fits \\
SN2012bo & A & J & 2012-04-02 & 56019 & -2 & SN2012bo\_A\_J\_20120402.fits \\
SN2012bp & A & H & 2012-04-02 & 56019 & 6 & SN2012bp\_A\_H\_20120402.fits \\
SN2012bp & A & J & 2012-04-02 & 56019 & 6 & SN2012bp\_A\_J\_20120402.fits \\
SN2012cg & A & H & 2013-04-25 & 56407 & 389 & SN2012cg\_A\_H\_20130425.fits \\
SN2012cg & A & H & 2013-05-23 & 56435 & 417 & SN2012cg\_A\_H\_20130523.fits \\
SN2012cg & A & H & 2013-05-28 & 56440 & 422 & SN2012cg\_A\_H\_20130528.fits \\
SN2012cg & A & H & 2013-06-13 & 56456 & 438 & SN2012cg\_A\_H\_20130613.fits \\
SN2012cg & A & H & 2013-06-17 & 56460 & 442 & SN2012cg\_A\_H\_20130617.fits \\
SN2012cg & A & J & 2013-04-25 & 56407 & 389 & SN2012cg\_A\_J\_20130425.fits \\
SN2012cg & A & J & 2013-05-23 & 56435 & 417 & SN2012cg\_A\_J\_20130523.fits \\
SN2012cg & A & J & 2013-05-28 & 56440 & 422 & SN2012cg\_A\_J\_20130528.fits \\
SN2012cg & A & J & 2013-06-17 & 56460 & 442 & SN2012cg\_A\_J\_20130617.fits \\
SN2012em & A & H & 2012-09-25 & 56195 & 14 & SN2012em\_A\_H\_20120925.fits \\
SN2012em & A & H & 2012-10-01 & 56201 & 20 & SN2012em\_A\_H\_20121001.fits \\
SN2012em & A & H & 2012-10-07 & 56207 & 26 & SN2012em\_A\_H\_20121007.fits \\
SN2012em & A & J & 2012-09-25 & 56195 & 14 & SN2012em\_A\_J\_20120925.fits \\
SN2012em & A & J & 2012-10-01 & 56201 & 20 & SN2012em\_A\_J\_20121001.fits \\
SN2012em & A & J & 2012-10-07 & 56207 & 26 & SN2012em\_A\_J\_20121007.fits \\
SN2012et & A & H & 2012-09-25 & 56195 & 9 & SN2012et\_A\_H\_20120925.fits \\
SN2012et & A & H & 2012-10-01 & 56201 & 15 & SN2012et\_A\_H\_20121001.fits \\
SN2012et & A & H & 2012-10-07 & 56207 & 21 & SN2012et\_A\_H\_20121007.fits \\
SN2012et & A & H & 2012-10-28 & 56228 & 42 & SN2012et\_A\_H\_20121028.fits \\
SN2012et & A & H & 2012-11-02 & 56233 & 47 & SN2012et\_A\_H\_20121102.fits \\
SN2012et & A & H & 2012-11-22 & 56253 & 67 & SN2012et\_A\_H\_20121122.fits \\
SN2012et & A & H & 2012-11-25 & 56256 & 70 & SN2012et\_A\_H\_20121125.fits \\
SN2012et & A & H & 2012-11-30 & 56261 & 75 & SN2012et\_A\_H\_20121130.fits \\
SN2012et & A & J & 2012-09-25 & 56195 & 9 & SN2012et\_A\_J\_20120925.fits \\
SN2012et & A & J & 2012-10-01 & 56201 & 15 & SN2012et\_A\_J\_20121001.fits \\
SN2012et & A & J & 2012-10-07 & 56207 & 21 & SN2012et\_A\_J\_20121007.fits \\
SN2012et & A & J & 2012-10-28 & 56228 & 42 & SN2012et\_A\_J\_20121028.fits \\
SN2012et & A & J & 2012-11-02 & 56233 & 47 & SN2012et\_A\_J\_20121102.fits \\
SN2012et & A & J & 2012-11-22 & 56253 & 67 & SN2012et\_A\_J\_20121122.fits \\
SN2012fb & A & H & 2012-09-25 & 56195 & 0 & SN2012fb\_A\_H\_20120925.fits \\
SN2012fb & A & H & 2012-10-01 & 56201 & 6 & SN2012fb\_A\_H\_20121001.fits \\
SN2012fb & A & H & 2012-10-07 & 56207 & 12 & SN2012fb\_A\_H\_20121007.fits \\
SN2012fb & A & J & 2012-09-25 & 56195 & 0 & SN2012fb\_A\_J\_20120925.fits \\
SN2012fb & A & J & 2012-10-01 & 56201 & 6 & SN2012fb\_A\_J\_20121001.fits \\
SN2012fb & A & J & 2012-10-07 & 56207 & 12 & SN2012fb\_A\_J\_20121007.fits \\
SN2012fk & A & H & 2012-11-02 & 56233 & 10 & SN2012fk\_A\_H\_20121102.fits \\
SN2012fk & A & H & 2012-11-22 & 56253 & 30 & SN2012fk\_A\_H\_20121122.fits \\
SN2012fk & A & H & 2012-11-25 & 56256 & 33 & SN2012fk\_A\_H\_20121125.fits \\
SN2012fk & A & H & 2012-11-30 & 56261 & 38 & SN2012fk\_A\_H\_20121130.fits \\
SN2012fk & A & J & 2012-11-02 & 56233 & 10 & SN2012fk\_A\_J\_20121102.fits \\
SN2012fk & A & J & 2012-11-22 & 56253 & 30 & SN2012fk\_A\_J\_20121122.fits \\
SN2012fk & A & J & 2012-11-25 & 56256 & 33 & SN2012fk\_A\_J\_20121125.fits \\
SN2012fk & A & J & 2012-11-30 & 56261 & 38 & SN2012fk\_A\_J\_20121130.fits \\
SN2012fm & A & H & 2012-10-28 & 56228 & 0 & SN2012fm\_A\_H\_20121028.fits \\
SN2012fm & A & H & 2012-11-02 & 56233 & 5 & SN2012fm\_A\_H\_20121102.fits \\
SN2012fm & A & H & 2012-11-22 & 56253 & 25 & SN2012fm\_A\_H\_20121122.fits \\
SN2012fm & A & H & 2012-11-25 & 56256 & 28 & SN2012fm\_A\_H\_20121125.fits \\
SN2012fm & A & H & 2012-11-30 & 56261 & 33 & SN2012fm\_A\_H\_20121130.fits \\
SN2012fm & A & H & 2013-10-18 & 56583 & 355 & SN2012fm\_A\_H\_20131018.fits \\
SN2012fm & A & J & 2012-10-28 & 56228 & 0 & SN2012fm\_A\_J\_20121028.fits \\
SN2012fm & A & J & 2012-11-02 & 56233 & 5 & SN2012fm\_A\_J\_20121102.fits \\
SN2012fm & A & J & 2012-11-22 & 56253 & 25 & SN2012fm\_A\_J\_20121122.fits \\
SN2012fm & A & J & 2012-11-25 & 56256 & 28 & SN2012fm\_A\_J\_20121125.fits \\
SN2012fm & A & J & 2012-11-30 & 56261 & 33 & SN2012fm\_A\_J\_20121130.fits \\
SN2012fm & A & J & 2013-10-18 & 56583 & 355 & SN2012fm\_A\_J\_20131018.fits \\
SN2012fr & A & H & 2012-11-02 & 56233 & -7 & SN2012fr\_A\_H\_20121102.fits \\
SN2012fr & A & J & 2012-11-02 & 56233 & -7 & SN2012fr\_A\_J\_20121102.fits \\
SN2012gm & A & H & 2012-11-22 & 56253 & -7 & SN2012gm\_A\_H\_20121122.fits \\
SN2012gm & A & H & 2012-11-25 & 56256 & -4 & SN2012gm\_A\_H\_20121125.fits \\
SN2012gm & A & H & 2012-11-30 & 56261 & 1 & SN2012gm\_A\_H\_20121130.fits \\
SN2012gm & A & J & 2012-11-22 & 56253 & -7 & SN2012gm\_A\_J\_20121122.fits \\
SN2012gm & A & J & 2012-11-25 & 56256 & -4 & SN2012gm\_A\_J\_20121125.fits \\
SN2012gm & A & J & 2012-11-30 & 56261 & 1 & SN2012gm\_A\_J\_20121130.fits \\
SN2012gm & A & KS & 2012-11-25 & 56256 & -4 & SN2012gm\_A\_KS\_20121125.fits \\
SN2012gm & A & KS & 2012-11-30 & 56261 & 1 & SN2012gm\_A\_KS\_20121130.fits \\
SN2012go & A & H & 2012-11-25 & 56256 & 4 & SN2012go\_A\_H\_20121125.fits \\
SN2012go & A & H & 2012-11-30 & 56261 & 9 & SN2012go\_A\_H\_20121130.fits \\
SN2012go & A & J & 2012-11-25 & 56256 & 4 & SN2012go\_A\_J\_20121125.fits \\
SN2012go & A & J & 2012-11-30 & 56261 & 9 & SN2012go\_A\_J\_20121130.fits \\
SN2013ar & A & H & 2013-03-26 & 56377 & 3 & SN2013ar\_A\_H\_20130326.fits \\
SN2013ar & A & H & 2013-04-20 & 56402 & 28 & SN2013ar\_A\_H\_20130420.fits \\
SN2013ar & A & H & 2013-04-29 & 56411 & 37 & SN2013ar\_A\_H\_20130429.fits \\
SN2013ar & A & J & 2013-03-26 & 56377 & 3 & SN2013ar\_A\_J\_20130326.fits \\
SN2013ar & A & J & 2013-04-20 & 56402 & 28 & SN2013ar\_A\_J\_20130420.fits \\
SN2013ar & A & J & 2013-04-29 & 56411 & 37 & SN2013ar\_A\_J\_20130429.fits \\
SN2013be & A & H & 2013-04-25 & 56407 & 9 & SN2013be\_A\_H\_20130425.fits \\
SN2013be & A & H & 2013-04-29 & 56411 & 13 & SN2013be\_A\_H\_20130429.fits \\
SN2013be & A & H & 2013-05-19 & 56431 & 33 & SN2013be\_A\_H\_20130519.fits \\
SN2013be & A & J & 2013-04-25 & 56407 & 9 & SN2013be\_A\_J\_20130425.fits \\
SN2013be & A & J & 2013-04-29 & 56411 & 13 & SN2013be\_A\_J\_20130429.fits \\
SN2013be & A & J & 2013-05-19 & 56431 & 33 & SN2013be\_A\_J\_20130519.fits \\
SN2013bo & A & H & 2013-04-20 & 56402 & 9 & SN2013bo\_A\_H\_20130420.fits \\
SN2013bo & A & H & 2013-04-25 & 56407 & 14 & SN2013bo\_A\_H\_20130425.fits \\
SN2013bo & A & H & 2013-04-29 & 56411 & 18 & SN2013bo\_A\_H\_20130429.fits \\
SN2013bo & A & H & 2013-05-22 & 56434 & 41 & SN2013bo\_A\_H\_20130522.fits \\
SN2013bo & A & J & 2013-04-20 & 56402 & 9 & SN2013bo\_A\_J\_20130420.fits \\
SN2013bo & A & J & 2013-04-25 & 56407 & 14 & SN2013bo\_A\_J\_20130425.fits \\
SN2013bo & A & J & 2013-04-29 & 56411 & 18 & SN2013bo\_A\_J\_20130429.fits \\
SN2013bo & A & J & 2013-05-22 & 56434 & 41 & SN2013bo\_A\_J\_20130522.fits \\
SN2013bq & A & H & 2013-04-20 & 56402 & -4 & SN2013bq\_A\_H\_20130420.fits \\
SN2013bq & A & H & 2013-04-25 & 56407 & 1 & SN2013bq\_A\_H\_20130425.fits \\
SN2013bq & A & H & 2013-05-23 & 56435 & 29 & SN2013bq\_A\_H\_20130523.fits \\
SN2013bq & A & J & 2013-04-20 & 56402 & -4 & SN2013bq\_A\_J\_20130420.fits \\
SN2013bq & A & J & 2013-04-25 & 56407 & 1 & SN2013bq\_A\_J\_20130425.fits \\
SN2013bq & A & J & 2013-04-29 & 56411 & 5 & SN2013bq\_A\_J\_20130429.fits \\
SN2013bs & A & H & 2013-04-20 & 56402 & -1 & SN2013bs\_A\_H\_20130420.fits \\
SN2013bs & A & H & 2013-04-25 & 56407 & 4 & SN2013bs\_A\_H\_20130425.fits \\
SN2013bs & A & H & 2013-04-29 & 56411 & 8 & SN2013bs\_A\_H\_20130429.fits \\
SN2013bs & A & H & 2013-05-22 & 56434 & 31 & SN2013bs\_A\_H\_20130522.fits \\
SN2013bs & A & H & 2013-05-28 & 56440 & 37 & SN2013bs\_A\_H\_20130528.fits \\
SN2013bs & A & H & 2013-06-13 & 56456 & 53 & SN2013bs\_A\_H\_20130613.fits \\
SN2013bs & A & H & 2013-06-17 & 56460 & 57 & SN2013bs\_A\_H\_20130617.fits \\
SN2013bs & A & J & 2013-04-20 & 56402 & -1 & SN2013bs\_A\_J\_20130420.fits \\
SN2013bs & A & J & 2013-04-25 & 56407 & 4 & SN2013bs\_A\_J\_20130425.fits \\
SN2013bs & A & J & 2013-05-22 & 56434 & 31 & SN2013bs\_A\_J\_20130522.fits \\
SN2013bs & A & J & 2013-05-28 & 56440 & 37 & SN2013bs\_A\_J\_20130528.fits \\
SN2013bs & A & J & 2013-06-13 & 56456 & 53 & SN2013bs\_A\_J\_20130613.fits \\
SN2013bs & A & J & 2013-06-17 & 56460 & 57 & SN2013bs\_A\_J\_20130617.fits \\
SN2013bt & A & H & 2013-04-20 & 56402 & -6 & SN2013bt\_A\_H\_20130420.fits \\
SN2013bt & A & H & 2013-04-25 & 56407 & -1 & SN2013bt\_A\_H\_20130425.fits \\
SN2013bt & A & H & 2013-04-29 & 56411 & 3 & SN2013bt\_A\_H\_20130429.fits \\
SN2013bt & A & H & 2013-05-19 & 56431 & 23 & SN2013bt\_A\_H\_20130519.fits \\
SN2013bt & A & H & 2013-05-23 & 56435 & 27 & SN2013bt\_A\_H\_20130523.fits \\
SN2013bt & A & J & 2013-04-20 & 56402 & -6 & SN2013bt\_A\_J\_20130420.fits \\
SN2013bt & A & J & 2013-04-25 & 56407 & -1 & SN2013bt\_A\_J\_20130425.fits \\
SN2013bt & A & J & 2013-04-29 & 56411 & 3 & SN2013bt\_A\_J\_20130429.fits \\
SN2013bt & A & J & 2013-05-19 & 56431 & 23 & SN2013bt\_A\_J\_20130519.fits \\
SN2013bt & A & J & 2013-05-23 & 56435 & 27 & SN2013bt\_A\_J\_20130523.fits \\
SN2013cb & A & H & 2013-05-19 & 56431 & 7 & SN2013cb\_A\_H\_20130519.fits \\
SN2013cb & A & H & 2013-05-23 & 56435 & 11 & SN2013cb\_A\_H\_20130523.fits \\
SN2013cb & A & H & 2013-05-28 & 56440 & 16 & SN2013cb\_A\_H\_20130528.fits \\
SN2013cb & A & J & 2013-05-19 & 56431 & 7 & SN2013cb\_A\_J\_20130519.fits \\
SN2013cb & A & J & 2013-05-23 & 56435 & 11 & SN2013cb\_A\_J\_20130523.fits \\
SN2013ck & A & H & 2013-05-19 & 56431 & 7 & SN2013ck\_A\_H\_20130519.fits \\
SN2013ck & A & H & 2013-05-23 & 56435 & 11 & SN2013ck\_A\_H\_20130523.fits \\
SN2013ck & A & H & 2013-06-13 & 56456 & 32 & SN2013ck\_A\_H\_20130613.fits \\
SN2013ck & A & H & 2013-06-17 & 56460 & 36 & SN2013ck\_A\_H\_20130617.fits \\
SN2013ck & A & J & 2013-05-19 & 56431 & 7 & SN2013ck\_A\_J\_20130519.fits \\
SN2013ck & A & J & 2013-05-23 & 56435 & 11 & SN2013ck\_A\_J\_20130523.fits \\
SN2013ck & A & J & 2013-06-13 & 56456 & 32 & SN2013ck\_A\_J\_20130613.fits \\
SN2013ck & A & J & 2013-06-17 & 56460 & 36 & SN2013ck\_A\_J\_20130617.fits \\
SN2013cs & A & H & 2013-05-23 & 56435 & -1 & SN2013cs\_A\_H\_20130523.fits \\
SN2013cs & A & H & 2013-05-28 & 56440 & 4 & SN2013cs\_A\_H\_20130528.fits \\
SN2013cs & A & H & 2013-06-13 & 56456 & 20 & SN2013cs\_A\_H\_20130613.fits \\
SN2013cs & A & H & 2013-06-17 & 56460 & 24 & SN2013cs\_A\_H\_20130617.fits \\
SN2013cs & A & J & 2013-05-23 & 56435 & -1 & SN2013cs\_A\_J\_20130523.fits \\
SN2013cs & A & J & 2013-05-28 & 56440 & 4 & SN2013cs\_A\_J\_20130528.fits \\
SN2013cs & A & J & 2013-06-13 & 56456 & 20 & SN2013cs\_A\_J\_20130613.fits \\
SN2013cs & A & J & 2013-06-17 & 56460 & 24 & SN2013cs\_A\_J\_20130617.fits \\
SN2013cs & A & KS & 2013-05-23 & 56435 & -1 & SN2013cs\_A\_KS\_20130523.fits \\
SN2013cs & A & KS & 2013-05-28 & 56440 & 4 & SN2013cs\_A\_KS\_20130528.fits \\
SN2013da & A & H & 2013-06-13 & 56456 & 7 & SN2013da\_A\_H\_20130613.fits \\
SN2013da & A & H & 2013-06-17 & 56460 & 11 & SN2013da\_A\_H\_20130617.fits \\
SN2013da & A & J & 2013-06-13 & 56456 & 7 & SN2013da\_A\_J\_20130613.fits \\
SN2013da & A & J & 2013-06-17 & 56460 & 11 & SN2013da\_A\_J\_20130617.fits \\
SN2013da & A & KS & 2013-06-13 & 56456 & 7 & SN2013da\_A\_KS\_20130613.fits \\
SN2013da & A & KS & 2013-06-17 & 56460 & 11 & SN2013da\_A\_KS\_20130617.fits \\
SN2013fj & A & H & 2013-09-25 & 56560 & 15 & SN2013fj\_A\_H\_20130925.fits \\
SN2013fj & A & H & 2013-10-15 & 56580 & 35 & SN2013fj\_A\_H\_20131015.fits \\
SN2013fj & A & H & 2013-10-20 & 56585 & 40 & SN2013fj\_A\_H\_20131020.fits \\
SN2013fj & A & J & 2013-09-25 & 56560 & 15 & SN2013fj\_A\_J\_20130925.fits \\
SN2013fj & A & J & 2013-10-15 & 56580 & 35 & SN2013fj\_A\_J\_20131015.fits \\
SN2013fj & A & J & 2013-10-20 & 56585 & 40 & SN2013fj\_A\_J\_20131020.fits \\
SN2013fn & A & H & 2013-10-15 & 56580 & 8 & SN2013fn\_A\_H\_20131015.fits \\
SN2013fn & A & H & 2013-10-20 & 56585 & 13 & SN2013fn\_A\_H\_20131020.fits \\
SN2013fn & A & H & 2013-11-11 & 56607 & 35 & SN2013fn\_A\_H\_20131111.fits \\
SN2013fn & A & J & 2013-10-15 & 56580 & 8 & SN2013fn\_A\_J\_20131015.fits \\
SN2013fn & A & J & 2013-10-20 & 56585 & 13 & SN2013fn\_A\_J\_20131020.fits \\
SN2013fn & A & J & 2013-11-11 & 56607 & 35 & SN2013fn\_A\_J\_20131111.fits \\
SN2013fn & A & KS & 2013-10-15 & 56580 & 8 & SN2013fn\_A\_KS\_20131015.fits \\
SN2013fn & A & KS & 2013-10-20 & 56585 & 13 & SN2013fn\_A\_KS\_20131020.fits \\
SN2013fw & A & H & 2013-11-11 & 56607 & 4 & SN2013fw\_A\_H\_20131111.fits \\
SN2013fw & A & H & 2013-11-20 & 56616 & 13 & SN2013fw\_A\_H\_20131120.fits \\
SN2013fw & A & H & 2013-12-09 & 56635 & 32 & SN2013fw\_A\_H\_20131209.fits \\
SN2013fw & A & H & 2013-12-13 & 56639 & 36 & SN2013fw\_A\_H\_20131213.fits \\
SN2013fw & A & J & 2013-11-11 & 56607 & 4 & SN2013fw\_A\_J\_20131111.fits \\
SN2013fw & A & J & 2013-11-20 & 56616 & 13 & SN2013fw\_A\_J\_20131120.fits \\
SN2013fw & A & J & 2013-12-09 & 56635 & 32 & SN2013fw\_A\_J\_20131209.fits \\
SN2013fw & A & J & 2013-12-13 & 56639 & 36 & SN2013fw\_A\_J\_20131213.fits \\
SN2013fw & A & KS & 2013-11-11 & 56607 & 4 & SN2013fw\_A\_KS\_20131111.fits \\
SN2013fw & A & KS & 2013-11-20 & 56616 & 13 & SN2013fw\_A\_KS\_20131120.fits \\
SN2013fw & A & KS & 2013-12-09 & 56635 & 32 & SN2013fw\_A\_KS\_20131209.fits \\
SN2013fw & A & KS & 2013-12-13 & 56639 & 36 & SN2013fw\_A\_KS\_20131213.fits \\
SNhunt175 & A & H & 2013-03-21 & 56372 & 3 & SNhunt175\_A\_H\_20130321.fits \\
SNhunt175 & A & H & 2013-04-20 & 56402 & 33 & SNhunt175\_A\_H\_20130420.fits \\
SNhunt175 & A & H & 2013-04-29 & 56411 & 42 & SNhunt175\_A\_H\_20130429.fits \\
SNhunt175 & A & J & 2013-04-20 & 56402 & 33 & SNhunt175\_A\_J\_20130420.fits \\
SNhunt206 & A & H & 2013-09-25 & 56560 & 12 & SNhunt206\_A\_H\_20130925.fits \\
SNhunt206 & A & H & 2013-09-27 & 56562 & 14 & SNhunt206\_A\_H\_20130927.fits \\
SNhunt206 & A & H & 2013-10-15 & 56580 & 32 & SNhunt206\_A\_H\_20131015.fits \\
SNhunt206 & A & H & 2013-10-20 & 56585 & 37 & SNhunt206\_A\_H\_20131020.fits \\
SNhunt206 & A & H & 2013-11-11 & 56607 & 59 & SNhunt206\_A\_H\_20131111.fits \\
SNhunt206 & A & J & 2013-09-25 & 56560 & 12 & SNhunt206\_A\_J\_20130925.fits \\
SNhunt206 & A & J & 2013-09-27 & 56562 & 14 & SNhunt206\_A\_J\_20130927.fits \\
SNhunt206 & A & J & 2013-10-15 & 56580 & 32 & SNhunt206\_A\_J\_20131015.fits \\
SNhunt206 & A & J & 2013-10-20 & 56585 & 37 & SNhunt206\_A\_J\_20131020.fits \\
SNhunt206 & A & J & 2013-11-11 & 56607 & 59 & SNhunt206\_A\_J\_20131111.fits \\
iPTF13dge & A & H & 2013-09-27 & 56562 & 7 & iPTF13dge\_A\_H\_20130927.fits \\
iPTF13dge & A & H & 2013-10-15 & 56580 & 25 & iPTF13dge\_A\_H\_20131015.fits \\
iPTF13dge & A & H & 2013-10-18 & 56583 & 28 & iPTF13dge\_A\_H\_20131018.fits \\
iPTF13dge & A & H & 2013-10-20 & 56585 & 30 & iPTF13dge\_A\_H\_20131020.fits \\
iPTF13dge & A & H & 2013-10-25 & 56590 & 35 & iPTF13dge\_A\_H\_20131025.fits \\
iPTF13dge & A & H & 2013-11-11 & 56607 & 52 & iPTF13dge\_A\_H\_20131111.fits \\
iPTF13dge & A & H & 2013-12-09 & 56635 & 80 & iPTF13dge\_A\_H\_20131209.fits \\
iPTF13dge & A & H & 2013-12-13 & 56639 & 84 & iPTF13dge\_A\_H\_20131213.fits \\
iPTF13dge & A & J & 2013-09-27 & 56562 & 7 & iPTF13dge\_A\_J\_20130927.fits \\
iPTF13dge & A & J & 2013-10-15 & 56580 & 25 & iPTF13dge\_A\_J\_20131015.fits \\
iPTF13dge & A & J & 2013-10-18 & 56583 & 28 & iPTF13dge\_A\_J\_20131018.fits \\
iPTF13dge & A & J & 2013-10-20 & 56585 & 30 & iPTF13dge\_A\_J\_20131020.fits \\
iPTF13dge & A & J & 2013-10-25 & 56590 & 35 & iPTF13dge\_A\_J\_20131025.fits \\
iPTF13dge & A & J & 2013-11-11 & 56607 & 52 & iPTF13dge\_A\_J\_20131111.fits \\
iPTF13dge & A & J & 2013-12-09 & 56635 & 80 & iPTF13dge\_A\_J\_20131209.fits \\
iPTF13dge & A & J & 2013-12-13 & 56639 & 84 & iPTF13dge\_A\_J\_20131213.fits \\
iPTF13dge & A & KS & 2013-09-27 & 56562 & 7 & iPTF13dge\_A\_KS\_20130927.fits \\
iPTF13dge & A & KS & 2013-10-15 & 56580 & 25 & iPTF13dge\_A\_KS\_20131015.fits \\
iPTF13dge & A & KS & 2013-10-18 & 56583 & 28 & iPTF13dge\_A\_KS\_20131018.fits \\
iPTF13dge & A & KS & 2013-10-20 & 56585 & 30 & iPTF13dge\_A\_KS\_20131020.fits \\
iPTF13dge & A & KS & 2013-10-25 & 56590 & 35 & iPTF13dge\_A\_KS\_20131025.fits \\
iPTF13dge & A & KS & 2013-12-09 & 56635 & 80 & iPTF13dge\_A\_KS\_20131209.fits \\
iPTF13dge & A & KS & 2013-12-13 & 56639 & 84 & iPTF13dge\_A\_KS\_20131213.fits \\
iPTF13dkj & A & H & 2013-09-25 & 56560 & 5 & iPTF13dkj\_A\_H\_20130925.fits \\
iPTF13dkj & A & H & 2013-09-27 & 56562 & 7 & iPTF13dkj\_A\_H\_20130927.fits \\
iPTF13dkj & A & H & 2013-10-15 & 56580 & 25 & iPTF13dkj\_A\_H\_20131015.fits \\
iPTF13dkj & A & H & 2013-10-19 & 56584 & 29 & iPTF13dkj\_A\_H\_20131019.fits \\
iPTF13dkj & A & H & 2013-10-25 & 56590 & 35 & iPTF13dkj\_A\_H\_20131025.fits \\
iPTF13dkj & A & J & 2013-09-25 & 56560 & 5 & iPTF13dkj\_A\_J\_20130925.fits \\
iPTF13dkj & A & J & 2013-09-27 & 56562 & 7 & iPTF13dkj\_A\_J\_20130927.fits \\
iPTF13dkj & A & J & 2013-10-15 & 56580 & 25 & iPTF13dkj\_A\_J\_20131015.fits \\
iPTF13dkj & A & J & 2013-10-19 & 56584 & 29 & iPTF13dkj\_A\_J\_20131019.fits \\
iPTF13dkj & A & J & 2013-10-25 & 56590 & 35 & iPTF13dkj\_A\_J\_20131025.fits \\
iPTF13dkl & A & H & 2013-09-27 & 56562 & 6 & iPTF13dkl\_A\_H\_20130927.fits \\
iPTF13dkl & A & H & 2013-10-18 & 56583 & 27 & iPTF13dkl\_A\_H\_20131018.fits \\
iPTF13dkl & A & H & 2013-10-20 & 56585 & 29 & iPTF13dkl\_A\_H\_20131020.fits \\
iPTF13dkl & A & J & 2013-09-27 & 56562 & 6 & iPTF13dkl\_A\_J\_20130927.fits \\
iPTF13dkl & A & J & 2013-10-18 & 56583 & 27 & iPTF13dkl\_A\_J\_20131018.fits \\
iPTF13dkl & A & J & 2013-10-20 & 56585 & 29 & iPTF13dkl\_A\_J\_20131020.fits \\
iPTF13dkx & A & H & 2013-09-27 & 56562 & 1 & iPTF13dkx\_A\_H\_20130927.fits \\
iPTF13dkx & A & H & 2013-10-15 & 56580 & 19 & iPTF13dkx\_A\_H\_20131015.fits \\
iPTF13dkx & A & H & 2013-10-19 & 56584 & 23 & iPTF13dkx\_A\_H\_20131019.fits \\
iPTF13dkx & A & H & 2013-11-11 & 56607 & 46 & iPTF13dkx\_A\_H\_20131111.fits \\
iPTF13dkx & A & J & 2013-09-27 & 56562 & 1 & iPTF13dkx\_A\_J\_20130927.fits \\
iPTF13dkx & A & J & 2013-10-15 & 56580 & 19 & iPTF13dkx\_A\_J\_20131015.fits \\
iPTF13dkx & A & J & 2013-10-19 & 56584 & 23 & iPTF13dkx\_A\_J\_20131019.fits \\
iPTF13dkx & A & J & 2013-11-11 & 56607 & 46 & iPTF13dkx\_A\_J\_20131111.fits \\
iPTF13ebh & A & H & 2013-11-20 & 56616 & -3 & iPTF13ebh\_A\_H\_20131120.fits \\
iPTF13ebh & A & H & 2013-12-09 & 56635 & 16 & iPTF13ebh\_A\_H\_20131209.fits \\
iPTF13ebh & A & H & 2013-12-13 & 56639 & 20 & iPTF13ebh\_A\_H\_20131213.fits \\
iPTF13ebh & A & J & 2013-11-20 & 56616 & -3 & iPTF13ebh\_A\_J\_20131120.fits \\
iPTF13ebh & A & J & 2013-12-09 & 56635 & 16 & iPTF13ebh\_A\_J\_20131209.fits \\
iPTF13ebh & A & J & 2013-12-13 & 56639 & 20 & iPTF13ebh\_A\_J\_20131213.fits \\
iPTF13ebh & A & KS & 2013-11-20 & 56616 & -3 & iPTF13ebh\_A\_KS\_20131120.fits \\
iPTF13ebh & A & KS & 2013-12-09 & 56635 & 16 & iPTF13ebh\_A\_KS\_20131209.fits \\
iPTF13ebh & A & KS & 2013-12-13 & 56639 & 20 & iPTF13ebh\_A\_KS\_20131213.fits \\
\enddata

\tablenotetext{a}{YYYY-MM-DD of local evening at KPNO (MST).}

\end{deluxetable}


==> stack_out.tex <==
\begin{deluxetable}{lll}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
\tablecaption{Stack Inspection\label{table:stackinspection}}
\tablehead{\colhead{imageName} & \colhead{stackUsable} & \colhead{wcsGood}}
\startdata
PTF11moy\_A\_H\_20111025.fits & Y & Y \\
PTF11moy\_A\_J\_20111025.fits & Y & Y \\
PTF11mty\_A\_H\_20111025.fits & Y & Y \\
PTF11mty\_A\_J\_20111025.fits & Y & Y \\
SN2011fe\_A\_H\_20111025.fits & Y & Y \\
SN2011fe\_A\_J\_20111025.fits & Y & Y \\
SN2011fe\_A\_KS\_20111025.fits & Y & Y \\
SN2011fs\_A\_H\_20111025.fits & Y & Y \\
SN2011fs\_A\_J\_20111025.fits & Y & Y \\
SN2011fs\_A\_KS\_20111025.fits & Y & Y \\
SN2011gf\_A\_H\_20111025.fits & Y & Y \\
SN2011gf\_A\_J\_20111025.fits & Y & Y \\
PTF11mty\_A\_H\_20111115.fits & Y & Y \\
PTF11mty\_A\_J\_20111115.fits & Y & Y \\
PTF11owc\_A\_H\_20111115.fits & Y & Y \\
PTF11owc\_A\_J\_20111115.fits & Y & Y \\
SN2011fs\_A\_H\_20111115.fits & Y & Y \\
SN2011fs\_A\_J\_20111115.fits & Y & Y \\
SN2011gf\_A\_H\_20111115.fits & Y & Y \\
SN2011gf\_A\_J\_20111115.fits & Y & Y \\
SN2011gy\_A\_H\_20111115.fits & Y & Y \\
SN2011gy\_A\_J\_20111115.fits & Y & Y \\
SN2011ha\_A\_H\_20111115.fits & Y & Y \\
SN2011ha\_A\_J\_20111115.fits & Y & Y \\
SN2011hb\_A\_H\_20111115.fits & Y & Y \\
SN2011hb\_A\_J\_20111115.fits & Y & Y \\
SN2011hk\_A\_H\_20111115.fits & Y & Y \\
SN2011hk\_A\_J\_20111115.fits & Y & Y \\
PTF11owc\_A\_H\_20111121.fits & Y & Y \\
PTF11owc\_A\_J\_20111121.fits & Y & Y \\
SN2011gy\_A\_H\_20111121.fits & Y & Y \\
SN2011gy\_A\_J\_20111121.fits & Y & Y \\
SN2011ha\_A\_H\_20111121.fits & Y & Y \\
SN2011ho\_A\_H\_20111121.fits & Y & Y \\
SN2011hr\_A\_H\_20111121.fits & Y & Y \\
SN2011hr\_A\_J\_20111121.fits & Y & Y \\
PTF11owc\_A\_H\_20111208.fits & Y & Y \\
PTF11owc\_A\_J\_20111208.fits & Y & Y \\
PTF11qmo\_A\_H\_20111208.fits & Y & Y \\
PTF11qmo\_A\_J\_20111208.fits & Y & Y \\
PTF11qpc\_A\_H\_20111208.fits & Y & Y \\
PTF11qri\_A\_H\_20111208.fits & Y & Y \\
PTF11qri\_A\_J\_20111208.fits & Y & Y \\
PTF11qzq\_A\_H\_20111208.fits & Y & Y \\
PTF11qzq\_A\_J\_20111208.fits & Y & Y \\
SN2011fs\_A\_H\_20111208.fits & Y & Y \\
SN2011fs\_A\_J\_20111208.fits & Y & Y \\
SN2011gf\_A\_H\_20111208.fits & Y & Y \\
SN2011gy\_A\_H\_20111208.fits & Y & Y \\
SN2011gy\_A\_J\_20111208.fits & Y & Y \\
SN2011hb\_A\_H\_20111208.fits & Y & Y \\
SN2011hb\_A\_J\_20111208.fits & Y & Y \\
SN2011hk\_A\_H\_20111208.fits & Y & Y \\
SN2011hk\_A\_J\_20111208.fits & Y & Y \\
SN2011ho\_A\_H\_20111208.fits & Y & Y \\
SN2011hr\_A\_H\_20111208.fits & Y & Y \\
SN2011hr\_A\_J\_20111208.fits & Y & Y \\
SN2011io\_A\_H\_20111208.fits & Y & Y \\
SN2011io\_A\_J\_20111208.fits & Y & Y \\
SN2011iu\_A\_H\_20111208.fits & Y & Y \\
SN2011iu\_A\_J\_20111208.fits & Y & Y \\
PTF11qmo\_A\_H\_20120108.fits & Y & Y \\
PTF11qmo\_A\_J\_20120108.fits & Y & Y \\
PTF11qpc\_A\_H\_20120108.fits & Y & Y \\
PTF11qri\_A\_H\_20120108.fits & Y & Y \\
PTF11qri\_A\_J\_20120108.fits & Y & Y \\
PTF11qzq\_A\_H\_20120108.fits & Y & Y \\
PTF11qzq\_A\_J\_20120108.fits & Y & Y \\
SN2011fs\_A\_H\_20120108.fits & Y & Y \\
SN2011fs\_A\_J\_20120108.fits & Y & Y \\
SN2011gy\_A\_H\_20120108.fits & Y & Y \\
SN2011gy\_A\_J\_20120108.fits & Y & Y \\
SN2011hb\_A\_H\_20120108.fits & Y & Y \\
SN2011hb\_A\_J\_20120108.fits & Y & Y \\
SN2011hk\_A\_H\_20120108.fits & Y & Y \\
SN2011hk\_A\_J\_20120108.fits & Y & Y \\
SN2011ho\_A\_H\_20120108.fits & Y & Y \\
SN2011hr\_A\_H\_20120108.fits & Y & Y \\
SN2011hr\_A\_J\_20120108.fits & Y & Y \\
SN2011iu\_A\_H\_20120108.fits & Y & Y \\
SN2011iu\_A\_J\_20120108.fits & Y & Y \\
PTF11owc\_A\_H\_20120402.fits & Y & Y \\
PTF11owc\_A\_J\_20120402.fits & Y & Y \\
PTF11qpc\_A\_H\_20120402.fits & Y & Y \\
SN2011fe\_A\_H\_20120402.fits & Y & Y \\
SN2011fe\_A\_J\_20120402.fits & Y & Y \\
SN2011gy\_A\_H\_20120402.fits & Y & Y \\
SN2011ho\_A\_H\_20120402.fits & Y & Y \\
SN2011hr\_A\_H\_20120402.fits & Y & Y \\
SN2011hr\_A\_J\_20120402.fits & Y & Y \\
SN2011iy\_A\_H\_20120402.fits & Y & Y \\
SN2011iy\_A\_J\_20120402.fits & Y & Y \\
SN2011jh\_A\_H\_20120402.fits & Y & Y \\
SN2011jh\_A\_J\_20120402.fits & Y & Y \\
SN2012bh\_A\_H\_20120402.fits & Y & Y \\
SN2012bh\_A\_J\_20120402.fits & Y & Y \\
SN2012bm\_A\_H\_20120402.fits & Y & Y \\
SN2012bm\_A\_J\_20120402.fits & Y & Y \\
SN2012bo\_A\_H\_20120402.fits & Y & Y \\
SN2012bo\_A\_J\_20120402.fits & Y & Y \\
SN2012bp\_A\_H\_20120402.fits & Y & Y \\
SN2012bp\_A\_J\_20120402.fits & Y & Y \\
PTF11mty\_A\_H\_20120925.fits & Y & Y \\
PTF12iiq\_A\_H\_20120925.fits & Y & Y \\
PTF12iiq\_A\_J\_20120925.fits & Y & Y \\
PTF12ikt\_A\_H\_20120925.fits & Y & Y \\
PTF12ikt\_A\_J\_20120925.fits & Y & Y \\
SN2011iu\_A\_H\_20120925.fits & Y & Y \\
SN2012em\_A\_H\_20120925.fits & Y & Y \\
SN2012em\_A\_J\_20120925.fits & Y & Y \\
SN2012et\_A\_H\_20120925.fits & Y & Y \\
SN2012et\_A\_J\_20120925.fits & Y & Y \\
SN2012fb\_A\_H\_20120925.fits & Y & Y \\
SN2012fb\_A\_J\_20120925.fits & Y & Y \\
PTF12iiq\_A\_H\_20121001.fits & Y & Y \\
PTF12iiq\_A\_J\_20121001.fits & Y & Y \\
PTF12ikt\_A\_H\_20121001.fits & Y & Y \\
PTF12ikt\_A\_J\_20121001.fits & Y & Y \\
SN2011iu\_A\_J\_20121001.fits & Y & Y \\
SN2012em\_A\_H\_20121001.fits & Y & Y \\
SN2012em\_A\_J\_20121001.fits & Y & Y \\
SN2012et\_A\_H\_20121001.fits & Y & Y \\
SN2012et\_A\_J\_20121001.fits & Y & Y \\
SN2012fb\_A\_H\_20121001.fits & Y & Y \\
SN2012fb\_A\_J\_20121001.fits & Y & Y \\
PTF11mty\_A\_J\_20121007.fits & Y & Y \\
PTF11qzq\_A\_H\_20121007.fits & Y & Y \\
PTF12iiq\_A\_H\_20121007.fits & Y & Y \\
PTF12iiq\_A\_J\_20121007.fits & Y & Y \\
PTF12ikt\_A\_H\_20121007.fits & Y & Y \\
PTF12ikt\_A\_J\_20121007.fits & Y & Y \\
SN2012em\_A\_H\_20121007.fits & Y & Y \\
SN2012em\_A\_J\_20121007.fits & Y & Y \\
SN2012et\_A\_H\_20121007.fits & Y & Y \\
SN2012et\_A\_J\_20121007.fits & Y & Y \\
SN2012fb\_A\_H\_20121007.fits & Y & Y \\
SN2012fb\_A\_J\_20121007.fits & Y & Y \\
CSS121006:232854+085452\_A\_H\_20121028.fits & Y & Y \\
CSS121009:011101-172841\_A\_H\_20121028.fits & Y & Y \\
CSS121009:011101-172841\_A\_J\_20121028.fits & Y & Y \\
Comet168P\_A\_H\_20121028.fits & Y & Y \\
Comet168P\_A\_J\_20121028.fits & Y & Y \\
Comet168P\_A\_KS\_20121028.fits & Y & Y \\
LSQ12fhs\_A\_H\_20121028.fits & Y & Y \\
LSQ12fhs\_A\_J\_20121028.fits & Y & Y \\
LSQ12fmx\_A\_H\_20121028.fits & Y & Y \\
LSQ12fmx\_A\_J\_20121028.fits & Y & Y \\
PS1-12bwh\_A\_H\_20121028.fits & Y & Y \\
PS1-12bwh\_A\_J\_20121028.fits & Y & Y \\
PSNJ07250042+2347030\_A\_H\_20121028.fits & Y & Y \\
PSNJ07250042+2347030\_A\_J\_20121028.fits & Y & Y \\
SN2011gy\_A\_H\_20121028.fits & Y & Y \\
SN2011gy\_A\_J\_20121028.fits & Y & Y \\
SN2012et\_A\_H\_20121028.fits & Y & Y \\
SN2012et\_A\_J\_20121028.fits & Y & Y \\
SN2012fm\_A\_H\_20121028.fits & Y & Y \\
SN2012fm\_A\_J\_20121028.fits & Y & Y \\
CSS121006:232854+085452\_A\_H\_20121102.fits & Y & Y \\
CSS121009:011101-172841\_A\_H\_20121102.fits & Y & Y \\
CSS121009:011101-172841\_A\_J\_20121102.fits & Y & Y \\
Comet168P\_A\_H\_20121102.fits & Y & Y \\
Comet168P\_A\_J\_20121102.fits & Y & Y \\
Comet168P\_A\_KS\_20121102.fits & Y & Y \\
LSQ12fhs\_A\_H\_20121102.fits & Y & Y \\
LSQ12fhs\_A\_J\_20121102.fits & Y & Y \\
LSQ12fmx\_A\_H\_20121102.fits & Y & Y \\
LSQ12fmx\_A\_J\_20121102.fits & Y & Y \\
LSQ12fuk\_A\_H\_20121102.fits & Y & Y \\
LSQ12fuk\_A\_J\_20121102.fits & Y & Y \\
PS1-12bwh\_A\_H\_20121102.fits & Y & Y \\
PS1-12bwh\_A\_J\_20121102.fits & Y & Y \\
PSNJ07250042+2347030\_A\_H\_20121102.fits & Y & Y \\
PSNJ07250042+2347030\_A\_J\_20121102.fits & Y & Y \\
SN2012et\_A\_H\_20121102.fits & Y & Y \\
SN2012et\_A\_J\_20121102.fits & Y & Y \\
SN2012fk\_A\_H\_20121102.fits & Y & Y \\
SN2012fk\_A\_J\_20121102.fits & Y & Y \\
SN2012fm\_A\_H\_20121102.fits & Y & Y \\
SN2012fm\_A\_J\_20121102.fits & Y & Y \\
SN2012fr\_A\_H\_20121102.fits & Y & Y \\
SN2012fr\_A\_J\_20121102.fits & Y & Y \\
P161-D\_A\_H\_20121102.fits & Y & Y \\
P161-D\_A\_J\_20121102.fits & Y & Y \\
CSS121114:090202+101800\_A\_H\_20121122.fits & Y & Y \\
CSS121114:090202+101800\_A\_J\_20121122.fits & Y & Y \\
LSQ12fhs\_A\_H\_20121122.fits & Y & Y \\
LSQ12fhs\_A\_J\_20121122.fits & Y & Y \\
LSQ12fmx\_A\_J\_20121122.fits & N & N \\
LSQ12fuk\_A\_H\_20121122.fits & Y & Y \\
LSQ12fuk\_A\_J\_20121122.fits & Y & Y \\
LSQ12gef\_A\_H\_20121122.fits & Y & Y \\
LSQ12gef\_A\_J\_20121122.fits & Y & Y \\
PS1-12bwh\_A\_H\_20121122.fits & Y & Y \\
PS1-12bwh\_A\_J\_20121122.fits & Y & Y \\
PSNJ07250042+2347030\_A\_H\_20121122.fits & Y & Y \\
PSNJ07250042+2347030\_A\_J\_20121122.fits & Y & Y \\
SN2012et\_A\_H\_20121122.fits & Y & Y \\
SN2012et\_A\_J\_20121122.fits & Y & Y \\
SN2012fk\_A\_H\_20121122.fits & Y & Y \\
SN2012fk\_A\_J\_20121122.fits & Y & Y \\
SN2012fm\_A\_H\_20121122.fits & Y & Y \\
SN2012fm\_A\_J\_20121122.fits & Y & Y \\
SN2012gm\_A\_H\_20121122.fits & Y & N \\
SN2012gm\_A\_J\_20121122.fits & Y & N \\
SN2012gm\_A\_KS\_20121122.fits & Y & -- \\
P161-D\_A\_H\_20121122.fits & Y & Y \\
P161-D\_A\_J\_20121122.fits & Y & Y \\
P161-D\_A\_KS\_20121122.fits & Y & Y \\
P525-E\_A\_H\_20121122.fits & Y & Y \\
P525-E\_A\_J\_20121122.fits & N & N \\
P525-E\_A\_KS\_20121122.fits & Y & Y \\
P525-E\_B\_H\_20121122.fits & Y & Y \\
P525-E\_B\_J\_20121122.fits & Y & Y \\
P525-E\_B\_KS\_20121122.fits & Y & Y \\
CSS121114:090202+101800\_A\_H\_20121125.fits & Y & Y \\
CSS121114:090202+101800\_A\_J\_20121125.fits & Y & Y \\
LSQ12fmx\_A\_H\_20121125.fits & Y & Y \\
LSQ12fuk\_A\_H\_20121125.fits & Y & Y \\
LSQ12fuk\_A\_J\_20121125.fits & Y & Y \\
LSQ12gef\_A\_H\_20121125.fits & Y & Y \\
LSQ12gef\_A\_J\_20121125.fits & Y & Y \\
PS1-12bwh\_A\_H\_20121125.fits & Y & Y \\
PS1-12bwh\_A\_J\_20121125.fits & Y & Y \\
PSNJ07250042+2347030\_A\_H\_20121125.fits & Y & Y \\
PSNJ07250042+2347030\_A\_J\_20121125.fits & Y & Y \\
PTF11owc\_A\_H\_20121125.fits & Y & Y \\
SN2012et\_A\_H\_20121125.fits & Y & Y \\
SN2012fk\_A\_H\_20121125.fits & Y & Y \\
SN2012fk\_A\_J\_20121125.fits & Y & Y \\
SN2012fm\_A\_H\_20121125.fits & Y & Y \\
SN2012fm\_A\_J\_20121125.fits & Y & Y \\
SN2012gm\_A\_H\_20121125.fits & Y & Y \\
SN2012gm\_A\_J\_20121125.fits & Y & Y \\
SN2012gm\_A\_KS\_20121125.fits & Y & Y \\
SN2012go\_A\_H\_20121125.fits & Y & Y \\
SN2012go\_A\_J\_20121125.fits & Y & Y \\
P161-D\_A\_H\_20121125.fits & Y & Y \\
P161-D\_A\_J\_20121125.fits & Y & Y \\
P161-D\_A\_KS\_20121125.fits & Y & Y \\
P161-D\_B\_H\_20121125.fits & Y & Y \\
P161-D\_B\_J\_20121125.fits & Y & Y \\
P161-D\_B\_KS\_20121125.fits & Y & Y \\
P161-D\_C\_H\_20121125.fits & Y & Y \\
P161-D\_C\_J\_20121125.fits & Y & Y \\
P525-E\_A\_H\_20121125.fits & Y & Y \\
P525-E\_A\_J\_20121125.fits & Y & Y \\
P525-E\_A\_KS\_20121125.fits & Y & Y \\
P525-E\_B\_H\_20121125.fits & Y & Y \\
P525-E\_B\_J\_20121125.fits & Y & Y \\
P525-E\_B\_KS\_20121125.fits & Y & Y \\
P525-E\_C\_H\_20121125.fits & Y & Y \\
P525-E\_C\_J\_20121125.fits & Y & Y \\
P525-E\_C\_KS\_20121125.fits & Y & Y \\
CSS121114:090202+101800\_A\_H\_20121130.fits & Y & Y \\
CSS121114:090202+101800\_A\_J\_20121130.fits & Y & Y \\
LSQ12fhs\_A\_H\_20121130.fits & Y & Y \\
LSQ12fhs\_A\_J\_20121130.fits & Y & Y \\
LSQ12fmx\_A\_H\_20121130.fits & Y & Y \\
LSQ12fuk\_A\_H\_20121130.fits & Y & Y \\
LSQ12fuk\_A\_J\_20121130.fits & Y & Y \\
LSQ12gef\_A\_H\_20121130.fits & Y & Y \\
PS1-12bwh\_A\_H\_20121130.fits & Y & Y \\
PS1-12bwh\_A\_J\_20121130.fits & Y & Y \\
PSNJ07250042+2347030\_A\_H\_20121130.fits & Y & Y \\
PSNJ07250042+2347030\_A\_J\_20121130.fits & Y & Y \\
SN2012et\_A\_H\_20121130.fits & Y & Y \\
SN2012fk\_A\_H\_20121130.fits & Y & Y \\
SN2012fk\_A\_J\_20121130.fits & Y & Y \\
SN2012fm\_A\_H\_20121130.fits & Y & Y \\
SN2012fm\_A\_J\_20121130.fits & Y & Y \\
SN2012gm\_A\_H\_20121130.fits & Y & Y \\
SN2012gm\_A\_J\_20121130.fits & Y & Y \\
SN2012gm\_A\_KS\_20121130.fits & Y & Y \\
SN2012go\_A\_H\_20121130.fits & Y & Y \\
SN2012go\_A\_J\_20121130.fits & Y & Y \\
P161-D\_A\_H\_20121130.fits & Y & Y \\
P161-D\_A\_J\_20121130.fits & Y & Y \\
P161-D\_A\_KS\_20121130.fits & Y & Y \\
P525-E\_A\_H\_20121130.fits & N & N \\
P525-E\_A\_J\_20121130.fits & N & N \\
P525-E\_A\_KS\_20121130.fits & Y & Y \\
P525-E\_B\_H\_20121130.fits & Y & Y \\
P525-E\_B\_J\_20121130.fits & Y & Y \\
P525-E\_B\_KS\_20121130.fits & Y & Y \\
SNhunt175\_A\_H\_20130321.fits & Y & Y \\
CSS130218:092354+385837\_A\_H\_20130326.fits & Y & Y \\
CSS130317:082848+293031\_A\_H\_20130326.fits & Y & Y \\
CSS130317:082848+293031\_A\_J\_20130326.fits & Y & Y \\
SN2013ar\_A\_H\_20130326.fits & Y & Y \\
SN2013ar\_A\_J\_20130326.fits & Y & Y \\
P212-C\_A\_J\_20130326.fits & Y & Y \\
P212-C\_A\_KS\_20130326.fits & N & N \\
CSS130218:092354+385837\_A\_H\_20130420.fits & Y & Y \\
CSS130317:082848+293031\_A\_H\_20130420.fits & Y & Y \\
CSS130317:082848+293031\_A\_J\_20130420.fits & Y & Y \\
SN2013ar\_A\_H\_20130420.fits & Y & Y \\
SN2013ar\_A\_J\_20130420.fits & Y & Y \\
SN2013bo\_A\_H\_20130420.fits & Y & Y \\
SN2013bo\_A\_J\_20130420.fits & Y & Y \\
SN2013bq\_A\_H\_20130420.fits & Y & Y \\
SN2013bq\_A\_J\_20130420.fits & Y & Y \\
SN2013bs\_A\_H\_20130420.fits & Y & Y \\
SN2013bs\_A\_J\_20130420.fits & Y & Y \\
SN2013bt\_A\_H\_20130420.fits & Y & Y \\
SN2013bt\_A\_J\_20130420.fits & Y & Y \\
SNhunt175\_A\_H\_20130420.fits & Y & Y \\
SNhunt175\_A\_J\_20130420.fits & Y & Y \\
P212-C\_A\_J\_20130420.fits & Y & Y \\
P212-C\_A\_KS\_20130420.fits & Y & Y \\
P212-C\_B\_H\_20130420.fits & Y & Y \\
P212-C\_B\_J\_20130420.fits & Y & Y \\
P212-C\_B\_KS\_20130420.fits & Y & Y \\
P212-C\_C\_H\_20130420.fits & Y & Y \\
P212-C\_C\_J\_20130420.fits & Y & Y \\
P212-C\_C\_KS\_20130420.fits & N & Y \\
CSS130218:092354+385837\_A\_H\_20130425.fits & Y & Y \\
CSS130317:082848+293031\_A\_H\_20130425.fits & Y & Y \\
CSS130317:082848+293031\_A\_J\_20130425.fits & Y & Y \\
SN2012cg\_A\_H\_20130425.fits & Y & Y \\
SN2012cg\_A\_J\_20130425.fits & Y & Y \\
SN2013be\_A\_H\_20130425.fits & Y & Y \\
SN2013be\_A\_J\_20130425.fits & Y & Y \\
SN2013bo\_A\_H\_20130425.fits & Y & Y \\
SN2013bo\_A\_J\_20130425.fits & Y & Y \\
SN2013bq\_A\_H\_20130425.fits & Y & Y \\
SN2013bq\_A\_J\_20130425.fits & Y & Y \\
SN2013bs\_A\_H\_20130425.fits & Y & Y \\
SN2013bs\_A\_J\_20130425.fits & Y & Y \\
SN2013bt\_A\_H\_20130425.fits & Y & Y \\
SN2013bt\_A\_J\_20130425.fits & Y & Y \\
P212-C\_A\_H\_20130425.fits & N & N \\
P212-C\_B\_H\_20130425.fits & Y & Y \\
P212-C\_B\_J\_20130425.fits & Y & Y \\
P212-C\_B\_KS\_20130425.fits & Y & Y \\
SN2013ar\_A\_H\_20130429.fits & Y & Y \\
SN2013ar\_A\_J\_20130429.fits & Y & Y \\
SN2013be\_A\_H\_20130429.fits & Y & Y \\
SN2013be\_A\_J\_20130429.fits & Y & Y \\
SN2013bo\_A\_H\_20130429.fits & Y & Y \\
SN2013bo\_A\_J\_20130429.fits & Y & Y \\
SN2013bq\_A\_H\_20130429.fits & Y & N \\
SN2013bq\_A\_J\_20130429.fits & N & N \\
SN2013bs\_A\_H\_20130429.fits & Y & Y \\
SN2013bt\_A\_H\_20130429.fits & Y & Y \\
SN2013bt\_A\_J\_20130429.fits & Y & Y \\
SNhunt175\_A\_H\_20130429.fits & Y & Y \\
P212-C\_A\_H\_20130429.fits & Y & Y \\
P212-C\_A\_J\_20130429.fits & Y & Y \\
P212-C\_B\_H\_20130429.fits & Y & Y \\
P212-C\_B\_J\_20130429.fits & Y & Y \\
P212-C\_B\_KS\_20130429.fits & Y & Y \\
PTF13ayw\_A\_H\_20130519.fits & Y & Y \\
PTF13ayw\_A\_J\_20130519.fits & Y & Y \\
SN2013be\_A\_H\_20130519.fits & Y & Y \\
SN2013be\_A\_J\_20130519.fits & Y & Y \\
SN2013bt\_A\_H\_20130519.fits & Y & Y \\
SN2013bt\_A\_J\_20130519.fits & Y & Y \\
SN2013cb\_A\_H\_20130519.fits & Y & Y \\
SN2013cb\_A\_J\_20130519.fits & Y & Y \\
SN2013ck\_A\_H\_20130519.fits & Y & Y \\
SN2013ck\_A\_J\_20130519.fits & Y & Y \\
P212-C\_A\_H\_20130519.fits & Y & Y \\
P212-C\_A\_J\_20130519.fits & Y & Y \\
P330-E\_A\_H\_20130519.fits & N & N \\
P330-E\_A\_J\_20130519.fits & Y & Y \\
P330-E\_A\_KS\_20130519.fits & Y & Y \\
PTF13asv\_A\_H\_20130522.fits & Y & Y \\
PTF13asv\_A\_J\_20130522.fits & N & N \\
SN2013bo\_A\_H\_20130522.fits & Y & Y \\
SN2013bo\_A\_J\_20130522.fits & Y & Y \\
SN2013bs\_A\_H\_20130522.fits & Y & Y \\
SN2013bs\_A\_J\_20130522.fits & Y & Y \\
P330-E\_A\_H\_20130522.fits & Y & Y \\
P330-E\_A\_J\_20130522.fits & Y & Y \\
P330-E\_A\_KS\_20130522.fits & Y & Y \\
P330-E\_B\_H\_20130522.fits & Y & Y \\
P330-E\_B\_J\_20130522.fits & Y & Y \\
P330-E\_B\_KS\_20130522.fits & Y & Y \\
SN2012cg\_A\_H\_20130523.fits & Y & Y \\
SN2012cg\_A\_J\_20130523.fits & Y & Y \\
SN2013bq\_A\_H\_20130523.fits & N & N \\
SN2013bt\_A\_H\_20130523.fits & Y & Y \\
SN2013bt\_A\_J\_20130523.fits & Y & Y \\
SN2013cb\_A\_H\_20130523.fits & Y & Y \\
SN2013cb\_A\_J\_20130523.fits & Y & Y \\
SN2013ck\_A\_H\_20130523.fits & Y & Y \\
SN2013ck\_A\_J\_20130523.fits & Y & Y \\
SN2013cs\_A\_H\_20130523.fits & Y & Y \\
SN2013cs\_A\_J\_20130523.fits & Y & Y \\
SN2013cs\_A\_KS\_20130523.fits & Y & Y \\
P330-E\_A\_H\_20130523.fits & Y & Y \\
P330-E\_A\_J\_20130523.fits & Y & Y \\
P330-E\_A\_KS\_20130523.fits & Y & Y \\
S791-C\_A\_H\_20130523.fits & Y & Y \\
S791-C\_A\_J\_20130523.fits & Y & Y \\
S791-C\_A\_KS\_20130523.fits & Y & Y \\
S791-C\_B\_H\_20130523.fits & Y & Y \\
S791-C\_B\_J\_20130523.fits & Y & Y \\
S791-C\_B\_KS\_20130523.fits & Y & Y \\
PTF13asv\_A\_H\_20130528.fits & Y & Y \\
PTF13asv\_A\_J\_20130528.fits & Y & Y \\
PTF13ayw\_A\_H\_20130528.fits & Y & Y \\
PTF13ayw\_A\_J\_20130528.fits & Y & Y \\
SN2012cg\_A\_H\_20130528.fits & Y & Y \\
SN2012cg\_A\_J\_20130528.fits & Y & Y \\
SN2013bs\_A\_H\_20130528.fits & Y & Y \\
SN2013bs\_A\_J\_20130528.fits & Y & Y \\
SN2013cb\_A\_H\_20130528.fits & Y & Y \\
SN2013cs\_A\_H\_20130528.fits & Y & Y \\
SN2013cs\_A\_J\_20130528.fits & Y & Y \\
SN2013cs\_A\_KS\_20130528.fits & Y & Y \\
P330-E\_A\_H\_20130528.fits & Y & Y \\
P330-E\_A\_J\_20130528.fits & Y & Y \\
P330-E\_A\_KS\_20130528.fits & Y & Y \\
P330-E\_B\_H\_20130528.fits & Y & Y \\
P330-E\_B\_J\_20130528.fits & Y & Y \\
P330-E\_B\_KS\_20130528.fits & Y & Y \\
S791-C\_A\_H\_20130528.fits & Y & Y \\
S791-C\_A\_J\_20130528.fits & Y & Y \\
S791-C\_A\_KS\_20130528.fits & Y & Y \\
S791-C\_B\_H\_20130528.fits & Y & Y \\
S791-C\_B\_J\_20130528.fits & Y & Y \\
S791-C\_B\_KS\_20130528.fits & Y & Y \\
PTF13asv\_A\_H\_20130613.fits & Y & Y \\
PTF13asv\_A\_J\_20130613.fits & N & Y \\
PTF13ayw\_A\_H\_20130613.fits & Y & Y \\
PTF13ayw\_A\_J\_20130613.fits & Y & Y \\
SN2012cg\_A\_H\_20130613.fits & Y & Y \\
SN2013bs\_A\_H\_20130613.fits & Y & Y \\
SN2013bs\_A\_J\_20130613.fits & Y & Y \\
SN2013ck\_A\_H\_20130613.fits & Y & Y \\
SN2013ck\_A\_J\_20130613.fits & Y & Y \\
SN2013cs\_A\_H\_20130613.fits & Y & Y \\
SN2013cs\_A\_J\_20130613.fits & Y & Y \\
SN2013cs\_A\_KS\_20130613.fits & Y & N \\
SN2013da\_A\_H\_20130613.fits & Y & Y \\
SN2013da\_A\_J\_20130613.fits & Y & Y \\
SN2013da\_A\_KS\_20130613.fits & Y & Y \\
P330-E\_A\_H\_20130613.fits & Y & Y \\
P330-E\_A\_J\_20130613.fits & Y & Y \\
P330-E\_A\_KS\_20130613.fits & Y & Y \\
S791-C\_A\_H\_20130613.fits & Y & Y \\
S791-C\_A\_J\_20130613.fits & Y & Y \\
S791-C\_A\_KS\_20130613.fits & Y & Y \\
PTF13asv\_A\_H\_20130617.fits & Y & Y \\
PTF13asv\_A\_J\_20130617.fits & Y & Y \\
PTF13ayw\_A\_H\_20130617.fits & Y & Y \\
PTF13ayw\_A\_J\_20130617.fits & Y & Y \\
SN2012cg\_A\_H\_20130617.fits & Y & Y \\
SN2012cg\_A\_J\_20130617.fits & Y & Y \\
SN2013bs\_A\_H\_20130617.fits & Y & Y \\
SN2013bs\_A\_J\_20130617.fits & Y & Y \\
SN2013ck\_A\_H\_20130617.fits & Y & Y \\
SN2013ck\_A\_J\_20130617.fits & Y & Y \\
SN2013cs\_A\_H\_20130617.fits & Y & Y \\
SN2013cs\_A\_J\_20130617.fits & Y & Y \\
SN2013cs\_A\_KS\_20130617.fits & Y & N \\
SN2013da\_A\_H\_20130617.fits & Y & Y \\
SN2013da\_A\_J\_20130617.fits & Y & Y \\
SN2013da\_A\_KS\_20130617.fits & Y & Y \\
P330-E\_B\_H\_20130617.fits & Y & Y \\
P330-E\_B\_J\_20130617.fits & Y & Y \\
P330-E\_B\_KS\_20130617.fits & Y & Y \\
P525-E\_A\_H\_20130617.fits & N & Y \\
S791-C\_A\_H\_20130617.fits & Y & Y \\
S791-C\_A\_J\_20130617.fits & Y & Y \\
S791-C\_A\_KS\_20130617.fits & Y & Y \\
PTF11qzq\_A\_J\_20130925.fits & Y & Y \\
PTF13dad\_A\_H\_20130925.fits & Y & Y \\
PTF13dad\_A\_J\_20130925.fits & Y & Y \\
PTF13ddg\_A\_H\_20130925.fits & Y & Y \\
SN2013fj\_A\_H\_20130925.fits & Y & Y \\
SN2013fj\_A\_J\_20130925.fits & Y & Y \\
SNhunt206\_A\_H\_20130925.fits & Y & Y \\
SNhunt206\_A\_J\_20130925.fits & Y & Y \\
iPTF13dkj\_A\_H\_20130925.fits & Y & Y \\
iPTF13dkj\_A\_J\_20130925.fits & Y & Y \\
P161-D\_A\_H\_20130925.fits & Y & Y \\
P161-D\_A\_J\_20130925.fits & Y & Y \\
P161-D\_A\_KS\_20130925.fits & Y & Y \\
P161-D\_B\_H\_20130925.fits & Y & Y \\
P161-D\_B\_J\_20130925.fits & Y & Y \\
P161-D\_B\_KS\_20130925.fits & Y & Y \\
P161-D\_C\_H\_20130925.fits & Y & Y \\
P161-D\_C\_J\_20130925.fits & Y & Y \\
P161-D\_C\_KS\_20130925.fits & Y & Y \\
P525-E\_A\_H\_20130925.fits & N & Y \\
SNhunt206\_A\_H\_20130927.fits & Y & Y \\
SNhunt206\_A\_J\_20130927.fits & Y & Y \\
iPTF13dge\_A\_H\_20130927.fits & Y & Y \\
iPTF13dge\_A\_J\_20130927.fits & Y & Y \\
iPTF13dge\_A\_KS\_20130927.fits & Y & Y \\
iPTF13dkj\_A\_H\_20130927.fits & Y & Y \\
iPTF13dkj\_A\_J\_20130927.fits & Y & Y \\
iPTF13dkl\_A\_H\_20130927.fits & Y & Y \\
iPTF13dkl\_A\_J\_20130927.fits & Y & Y \\
iPTF13dkx\_A\_H\_20130927.fits & Y & Y \\
iPTF13dkx\_A\_J\_20130927.fits & Y & Y \\
P161-D\_A\_H\_20130927.fits & Y & Y \\
P161-D\_A\_J\_20130927.fits & Y & Y \\
P161-D\_A\_KS\_20130927.fits & Y & Y \\
P161-D\_B\_H\_20130927.fits & Y & Y \\
P161-D\_B\_J\_20130927.fits & Y & Y \\
P161-D\_B\_KS\_20130927.fits & Y & Y \\
P161-D\_C\_H\_20130927.fits & Y & Y \\
P161-D\_C\_J\_20130927.fits & Y & Y \\
P161-D\_C\_KS\_20130927.fits & Y & Y \\
P525-E\_A\_H\_20130927.fits & Y & Y \\
P525-E\_A\_J\_20130927.fits & Y & Y \\
P525-E\_A\_KS\_20130927.fits & Y & Y \\
P525-E\_B\_H\_20130927.fits & Y & Y \\
P525-E\_B\_J\_20130927.fits & Y & Y \\
P525-E\_B\_KS\_20130927.fits & N & N \\
P525-E\_C\_H\_20130927.fits & Y & Y \\
P525-E\_C\_J\_20130927.fits & Y & Y \\
P525-E\_C\_KS\_20130927.fits & Y & Y \\
LSQ13cmt\_A\_H\_20131015.fits & Y & Y \\
LSQ13cmt\_A\_J\_20131015.fits & Y & Y \\
PTF13dad\_A\_H\_20131015.fits & Y & Y \\
PTF13dad\_A\_J\_20131015.fits & Y & Y \\
PTF13ddg\_A\_H\_20131015.fits & Y & Y \\
SN2013fj\_A\_H\_20131015.fits & Y & Y \\
SN2013fj\_A\_J\_20131015.fits & Y & Y \\
SN2013fn\_A\_H\_20131015.fits & Y & Y \\
SN2013fn\_A\_J\_20131015.fits & Y & Y \\
SN2013fn\_A\_KS\_20131015.fits & Y & Y \\
SNhunt206\_A\_H\_20131015.fits & Y & Y \\
SNhunt206\_A\_J\_20131015.fits & Y & Y \\
iPTF13dge\_A\_H\_20131015.fits & Y & Y \\
iPTF13dge\_A\_J\_20131015.fits & Y & Y \\
iPTF13dge\_A\_KS\_20131015.fits & Y & Y \\
iPTF13dkj\_A\_H\_20131015.fits & Y & Y \\
iPTF13dkj\_A\_J\_20131015.fits & Y & Y \\
iPTF13dkx\_A\_H\_20131015.fits & Y & Y \\
iPTF13dkx\_A\_J\_20131015.fits & Y & Y \\
P161-D\_A\_H\_20131015.fits & Y & Y \\
P161-D\_A\_J\_20131015.fits & Y & Y \\
P161-D\_A\_KS\_20131015.fits & Y & Y \\
P161-D\_B\_H\_20131015.fits & Y & Y \\
P161-D\_B\_J\_20131015.fits & Y & Y \\
P161-D\_B\_KS\_20131015.fits & Y & Y \\
P161-D\_C\_H\_20131015.fits & Y & Y \\
P161-D\_C\_J\_20131015.fits & Y & Y \\
P161-D\_C\_KS\_20131015.fits & Y & Y \\
P525-E\_A\_H\_20131015.fits & Y & Y \\
P525-E\_A\_J\_20131015.fits & Y & Y \\
P525-E\_A\_KS\_20131015.fits & Y & Y \\
P525-E\_B\_H\_20131015.fits & Y & Y \\
P525-E\_B\_J\_20131015.fits & Y & Y \\
P525-E\_B\_KS\_20131015.fits & Y & Y \\
P525-E\_C\_H\_20131015.fits & Y & Y \\
P525-E\_C\_J\_20131015.fits & Y & Y \\
P525-E\_C\_KS\_20131015.fits & Y & Y \\
S840-F\_A\_H\_20131015.fits & Y & Y \\
S840-F\_A\_J\_20131015.fits & Y & Y \\
S840-F\_A\_KS\_20131015.fits & Y & Y \\
LSQ13cmt\_A\_H\_20131018.fits & Y & Y \\
PS1-13dkh\_A\_H\_20131018.fits & Y & Y \\
PS1-13dkh\_A\_J\_20131018.fits & Y & Y \\
SN2012fm\_A\_H\_20131018.fits & Y & Y \\
SN2012fm\_A\_J\_20131018.fits & Y & Y \\
iPTF13dge\_A\_H\_20131018.fits & Y & Y \\
iPTF13dge\_A\_J\_20131018.fits & Y & Y \\
iPTF13dge\_A\_KS\_20131018.fits & Y & Y \\
iPTF13dkl\_A\_H\_20131018.fits & Y & Y \\
iPTF13dkl\_A\_J\_20131018.fits & Y & Y \\
P161-D\_A\_H\_20131018.fits & Y & Y \\
P161-D\_A\_J\_20131018.fits & Y & Y \\
P161-D\_A\_KS\_20131018.fits & Y & Y \\
P161-D\_B\_H\_20131018.fits & Y & Y \\
P161-D\_B\_J\_20131018.fits & Y & Y \\
P161-D\_B\_KS\_20131018.fits & Y & Y \\
LSQ12fuk\_A\_H\_20131019.fits & Y & Y \\
LSQ12fuk\_A\_J\_20131019.fits & Y & Y \\
PTF13ddg\_A\_H\_20131019.fits & Y & Y \\
iPTF13dkj\_A\_H\_20131019.fits & Y & Y \\
iPTF13dkj\_A\_J\_20131019.fits & Y & Y \\
iPTF13dkx\_A\_H\_20131019.fits & Y & Y \\
iPTF13dkx\_A\_J\_20131019.fits & Y & Y \\
P525-E\_A\_H\_20131019.fits & Y & Y \\
P525-E\_A\_J\_20131019.fits & Y & Y \\
P525-E\_A\_KS\_20131019.fits & Y & Y \\
P525-E\_B\_H\_20131019.fits & Y & Y \\
P525-E\_B\_J\_20131019.fits & Y & Y \\
P525-E\_B\_KS\_20131019.fits & Y & Y \\
P525-E\_C\_H\_20131019.fits & Y & Y \\
P525-E\_C\_J\_20131019.fits & Y & Y \\
P525-E\_C\_KS\_20131019.fits & Y & Y \\
LSQ13cmt\_A\_H\_20131020.fits & Y & Y \\
LSQ13cmt\_A\_J\_20131020.fits & Y & Y \\
PTF13dad\_A\_H\_20131020.fits & Y & Y \\
PTF13dad\_A\_J\_20131020.fits & Y & Y \\
SN2011hb\_A\_H\_20131020.fits & Y & Y \\
SN2011hb\_A\_J\_20131020.fits & Y & Y \\
SN2013fj\_A\_H\_20131020.fits & N & Y \\
SN2013fj\_A\_J\_20131020.fits & Y & Y \\
SN2013fn\_A\_H\_20131020.fits & Y & Y \\
SN2013fn\_A\_J\_20131020.fits & Y & Y \\
SN2013fn\_A\_KS\_20131020.fits & Y & Y \\
SNhunt206\_A\_H\_20131020.fits & Y & Y \\
SNhunt206\_A\_J\_20131020.fits & Y & Y \\
iPTF13dge\_A\_H\_20131020.fits & Y & Y \\
iPTF13dge\_A\_J\_20131020.fits & Y & Y \\
iPTF13dge\_A\_KS\_20131020.fits & Y & Y \\
iPTF13dkl\_A\_H\_20131020.fits & N & Y \\
iPTF13dkl\_A\_J\_20131020.fits & Y & Y \\
P161-D\_A\_H\_20131020.fits & Y & Y \\
P161-D\_A\_J\_20131020.fits & Y & Y \\
P161-D\_A\_KS\_20131020.fits & Y & Y \\
P161-D\_B\_H\_20131020.fits & Y & Y \\
P161-D\_B\_J\_20131020.fits & Y & Y \\
P161-D\_B\_KS\_20131020.fits & Y & Y \\
P161-D\_C\_H\_20131020.fits & Y & Y \\
P161-D\_C\_J\_20131020.fits & Y & Y \\
P161-D\_C\_KS\_20131020.fits & Y & Y \\
P525-E\_A\_H\_20131020.fits & Y & Y \\
P525-E\_A\_J\_20131020.fits & Y & Y \\
P525-E\_A\_KS\_20131020.fits & Y & Y \\
P525-E\_B\_H\_20131020.fits & Y & Y \\
P525-E\_B\_J\_20131020.fits & Y & Y \\
P525-E\_B\_KS\_20131020.fits & Y & Y \\
P525-E\_C\_H\_20131020.fits & Y & Y \\
P525-E\_C\_J\_20131020.fits & N & N \\
P525-E\_C\_KS\_20131020.fits & N & N \\
LSQ13crf\_A\_H\_20131025.fits & Y & Y \\
LSQ13crf\_A\_J\_20131025.fits & Y & Y \\
SNhunt206\_A\_H\_20131025.fits & Y & Y \\
SNhunt206\_A\_J\_20131025.fits & Y & Y \\
iPTF13dge\_A\_H\_20131025.fits & Y & Y \\
iPTF13dge\_A\_J\_20131025.fits & Y & Y \\
iPTF13dge\_A\_KS\_20131025.fits & Y & Y \\
iPTF13dkj\_A\_H\_20131025.fits & Y & Y \\
iPTF13dkj\_A\_J\_20131025.fits & Y & Y \\
iPTF13dkl\_A\_H\_20131025.fits & Y & N \\
iPTF13dkx\_A\_H\_20131025.fits & Y & Y \\
iPTF13dkx\_A\_J\_20131025.fits & Y & N \\
P161-D\_A\_H\_20131025.fits & Y & Y \\
P161-D\_A\_J\_20131025.fits & Y & Y \\
P161-D\_A\_KS\_20131025.fits & Y & Y \\
P161-D\_B\_H\_20131025.fits & Y & Y \\
P161-D\_B\_J\_20131025.fits & Y & Y \\
P161-D\_B\_KS\_20131025.fits & Y & Y \\
LSQ13crf\_A\_H\_20131111.fits & Y & Y \\
LSQ13crf\_A\_J\_20131111.fits & Y & Y \\
LSQ13cwp\_A\_H\_20131111.fits & Y & Y \\
LSQ13cwp\_A\_J\_20131111.fits & Y & Y \\
PS1-13dkh\_A\_H\_20131111.fits & Y & Y \\
PS1-13dkh\_A\_J\_20131111.fits & Y & Y \\
SN2013fn\_A\_H\_20131111.fits & Y & Y \\
SN2013fn\_A\_J\_20131111.fits & Y & Y \\
SN2013fw\_A\_H\_20131111.fits & Y & Y \\
SN2013fw\_A\_J\_20131111.fits & Y & Y \\
SN2013fw\_A\_KS\_20131111.fits & Y & Y \\
SNhunt206\_A\_H\_20131111.fits & Y & Y \\
SNhunt206\_A\_J\_20131111.fits & Y & Y \\
iPTF13dge\_A\_H\_20131111.fits & Y & Y \\
iPTF13dge\_A\_J\_20131111.fits & Y & Y \\
iPTF13dkx\_A\_H\_20131111.fits & Y & Y \\
iPTF13dkx\_A\_J\_20131111.fits & Y & Y \\
P161-D\_A\_H\_20131111.fits & Y & Y \\
P161-D\_A\_J\_20131111.fits & Y & Y \\
P161-D\_A\_KS\_20131111.fits & Y & Y \\
P161-D\_B\_H\_20131111.fits & Y & Y \\
P161-D\_B\_J\_20131111.fits & Y & Y \\
P161-D\_B\_KS\_20131111.fits & Y & Y \\
P525-E\_A\_H\_20131111.fits & Y & Y \\
P525-E\_A\_J\_20131111.fits & Y & Y \\
P525-E\_A\_KS\_20131111.fits & Y & Y \\
P525-E\_B\_H\_20131111.fits & Y & Y \\
P525-E\_B\_J\_20131111.fits & Y & Y \\
P525-E\_B\_KS\_20131111.fits & Y & Y \\
P525-E\_C\_H\_20131111.fits & Y & Y \\
P525-E\_C\_J\_20131111.fits & Y & Y \\
P525-E\_C\_KS\_20131111.fits & Y & Y \\
LSQ13cwp\_A\_H\_20131120.fits & Y & Y \\
LSQ13cwp\_A\_J\_20131120.fits & Y & Y \\
PS1-13dkh\_A\_H\_20131120.fits & Y & Y \\
PS1-13dkh\_A\_J\_20131120.fits & Y & Y \\
SN2013fw\_A\_H\_20131120.fits & Y & Y \\
SN2013fw\_A\_J\_20131120.fits & Y & Y \\
SN2013fw\_A\_KS\_20131120.fits & Y & Y \\
iPTF13ebh\_A\_H\_20131120.fits & Y & Y \\
iPTF13ebh\_A\_J\_20131120.fits & Y & Y \\
iPTF13ebh\_A\_KS\_20131120.fits & Y & Y \\
P525-E\_A\_H\_20131120.fits & N & Y \\
LSQ13crf\_A\_H\_20131209.fits & Y & Y \\
LSQ13crf\_A\_J\_20131209.fits & Y & Y \\
LSQ13cwp\_A\_H\_20131209.fits & Y & Y \\
LSQ13cwp\_A\_J\_20131209.fits & Y & Y \\
PS1-13dkh\_A\_H\_20131209.fits & Y & Y \\
PS1-13dkh\_A\_J\_20131209.fits & Y & Y \\
SN2013fw\_A\_H\_20131209.fits & Y & Y \\
SN2013fw\_A\_J\_20131209.fits & Y & Y \\
SN2013fw\_A\_KS\_20131209.fits & Y & Y \\
iPTF13dge\_A\_H\_20131209.fits & Y & Y \\
iPTF13dge\_A\_J\_20131209.fits & Y & Y \\
iPTF13dge\_A\_KS\_20131209.fits & Y & Y \\
iPTF13ebh\_A\_H\_20131209.fits & Y & Y \\
iPTF13ebh\_A\_J\_20131209.fits & Y & Y \\
iPTF13ebh\_A\_KS\_20131209.fits & Y & Y \\
P161-D\_A\_H\_20131209.fits & Y & Y \\
P161-D\_A\_J\_20131209.fits & Y & Y \\
P161-D\_A\_KS\_20131209.fits & Y & Y \\
P161-D\_B\_H\_20131209.fits & Y & Y \\
P161-D\_B\_J\_20131209.fits & Y & Y \\
P161-D\_B\_KS\_20131209.fits & Y & Y \\
P525-E\_A\_H\_20131209.fits & Y & Y \\
P525-E\_A\_J\_20131209.fits & Y & Y \\
P525-E\_A\_KS\_20131209.fits & Y & Y \\
P525-E\_B\_H\_20131209.fits & Y & Y \\
P525-E\_B\_J\_20131209.fits & Y & Y \\
P525-E\_B\_KS\_20131209.fits & Y & Y \\
LSQ13crf\_A\_H\_20131213.fits & Y & Y \\
LSQ13cwp\_A\_H\_20131213.fits & Y & Y \\
LSQ13cwp\_A\_J\_20131213.fits & Y & Y \\
PSNJ07250042+2347030\_A\_H\_20131213.fits & Y & Y \\
PSNJ07250042+2347030\_A\_J\_20131213.fits & Y & Y \\
SN2011hr\_A\_H\_20131213.fits & Y & Y \\
SN2013fw\_A\_H\_20131213.fits & Y & Y \\
SN2013fw\_A\_J\_20131213.fits & Y & Y \\
SN2013fw\_A\_KS\_20131213.fits & Y & Y \\
iPTF13dge\_A\_H\_20131213.fits & Y & Y \\
iPTF13dge\_A\_J\_20131213.fits & Y & Y \\
iPTF13dge\_A\_KS\_20131213.fits & Y & Y \\
iPTF13ebh\_A\_H\_20131213.fits & Y & Y \\
iPTF13ebh\_A\_J\_20131213.fits & Y & Y \\
iPTF13ebh\_A\_KS\_20131213.fits & Y & Y \\
P161-D\_A\_H\_20131213.fits & Y & Y \\
P161-D\_A\_J\_20131213.fits & Y & Y \\
P161-D\_A\_KS\_20131213.fits & Y & Y \\
P161-D\_B\_H\_20131213.fits & Y & Y \\
P161-D\_B\_J\_20131213.fits & Y & Y \\
P161-D\_B\_KS\_20131213.fits & Y & Y \\
P525-E\_A\_H\_20131213.fits & Y & Y \\
P525-E\_A\_J\_20131213.fits & Y & Y \\
P525-E\_A\_KS\_20131213.fits & Y & Y \\
P525-E\_B\_H\_20131213.fits & Y & Y \\
P525-E\_B\_J\_20131213.fits & Y & Y \\
P525-E\_B\_KS\_20131213.fits & Y & Y
\enddata
 97.3\% of the stacks are usable.
 97.2\% of the stacks have good WCS.
 96.2\% of the stacks are usable and have good WCS.
Note that there a few stacks that are not usable but have good WCS:
e.g., the stack may have ended up with only one constituent raw image
and so have many masked regions, but has a good WCS solution.
\end{deluxetable}

